Near-optimal fitting of ellipsoids to random points

Given independent standard Gaussian points $v_1, \ldots, v_n$ in dimension $d$, for what values of $(n, d)$ does there exist with high probability an origin-symmetric ellipsoid that simultaneously passes through all of the points? This basic problem of fitting an ellipsoid to random points has connections to low-rank matrix decompositions, independent component analysis, and principal component analysis. Based on strong numerical evidence, Saunderson, Parrilo, and Willsky [Proc. of Conference on Decision and Control, pp. 6031-6036, 2013] conjecture that the ellipsoid fitting problem transitions from feasible to infeasible as the number of points $n$ increases, with a sharp threshold at $n \sim d^2/4$. We resolve this conjecture up to logarithmic factors by constructing a fitting ellipsoid for some $n = \Omega( \, d^2/\mathrm{polylog}(d) \,)$, improving prior work of Ghosh et al. [Proc. of Symposium on Foundations of Computer Science, pp. 954-965, 2020] that requires $n = o(d^{3/2})$. Our proof demonstrates feasibility of the least squares construction of Saunderson et al. using a convenient decomposition of a certain non-standard random matrix and a careful analysis of its Neumann expansion via the theory of graph matrices.

==> Notes/ellipsoid-fitting.tex <==
\section{Notation}
$I_d$ denotes the $d \times d$ identity matrix and $1_d$ denotes the all-ones vector in $\R^d$. For vectors $u,v$, $u \otimes v$ denotes the tensor (Kronecker) product of $u$ and $v$. For a linear operator $A: X \rightarrow Y$ between two normed spaces $(X,  \norm{\cdot}_X)$ and $(Y, \norm{\cdot}_Y)$, we define the following norm:
\[
\norm{A}_{X \rightarrow Y} = \sup_{x \in X,\, \norm{x}_X = 1} \norm{Ax}_Y.
\]
For the special case of $(\R^n, \norm{\cdot}_2)$ and $(\R^m, \norm{\cdot}_2)$, we use the notation $\norm{A}_{op}$. Define $A^\dagger$ be the pseudo-inverse of $A$ and $A^*$ its Hermitian adjoint. When the operator $AA^*$ is invertible, we have the expression $A^\dagger = A^* (AA^*)^{-1}$.

We use $\calN(0,I_d)$ to denote the standard Gaussian distribution on $\R^d$ and $\chi^2_d$ to denote the chi-squared distribution with $d$ degrees of freedom. Throughout, we let $v_1, \ldots, v_n \sim \calN(0, I_d)$ unless declared otherwise. We think of $n = n(d)$ as a function of $d$ and say an event holds ``with high probability'' (or w.h.p.)\ if it holds with probability tending to 1 as $d \rightarrow \infty$. Following~\cite{vershynin2018high}, call a random variable $X$ \emph{sub-gaussian} (or \emph{sub-exponential}) with parameter $K > 0$ if for all $t \geq 0$, it holds that $\Prob (|X| \geq t) \leq 2 \exp(-t^2/K^2)$ (or $\Prob (|X| \geq t) \leq 2 \exp(-t/K)$).

Define the linear operator $\calA : \R^{d \times d} \rightarrow \R^n$ by $\calA(X) = (v_1^T X v_1, \ldots, v_n^T X v_n)^T$. Then $\calA^* : \R^{n} \rightarrow \R^{d \times d}$ satisfies $\calA^* (c) = \sum_{i=1}^n c_i v_i v_i^T$. We identify $\calA \calA^*: \R^n \rightarrow \R^{n}$ with its representation as an $n \times n$ matrix that satisfies $(\calA \calA^*)_{ij} = \ip{v_i}{v_j}^2$ for $i,j \in [n]$. Finally, define $M = (d^2 -d)I_n + d 1_n 1_n^T$. It can be directly verified that $M^{-1} = \frac{1}{d(d-1)}(I_n - \frac{1}{n+d-1} 1_n 1_n^T)$, $M^{-1/2} = \frac{1}{\sqrt{d^2-d}} (I_n - \frac{1}{n} 1_n 1_n^T) + \frac{1}{n \sqrt{d (n+d-1)}} 1_n 1_n^T$, and $M^{-1/2} 1_n = \frac{1}{\sqrt{d (n+d-1)}} 1_n$.

\section{Proof of Theorem~\ref{thm:main}}
\label{sec:main-proof}

Before beginning the proof of the main theorem, we state the two key technical results used in the proof. The proofs of Propositions~\ref{prop:delta-norm} and~\ref{prop:delta-ones-vector} occupy Sections~\ref{sec:convergence-criterion} and~\ref{sec:delta-ones-vector}, respectively.
\begin{prop}
\label{prop:delta-norm}
With high probability, $\norm{M^{-1/2} \Delta M^{-1/2}}_{op} = O(\frac{\sqrt{n} \log^2 (n)}{d} + \frac{n \log^3 (dn)}{d^2}) + o(1)$.
\end{prop}

\begin{prop}
\label{prop:delta-ones-vector}
With high probability, $\norm{\Delta 1_n}_{\infty} = O(d \sqrt{n \log n} + \sqrt{dn} \log (n))$.
\end{prop}

\begin{proof}[Proof of Theorem~\ref{thm:main}]
As discussed in Section~\ref{sec:technical-overview}, it suffices to show that $X = X_{\text{LS}} \succeq 0$. While the high-level structure of our proof follows that of \cite{saunderson2011subspace,saunderson_parrilo_willsky13}, we explicitly write out the details since we work with $M^{-1/2} \Delta M^{-1/2}$ instead of $M^{-1} \Delta$. By monotonicity (with respect to $n$) of the probability of the ellipsoid fitting property holding, it suffices to fix $n = cd^2/\log^5 (d)$ for some constant $c > 0$ to be determined later. We proceed to showing $X \succeq 0$ by expanding $(\calA \calA^*)^{-1}$ as a Neumann series. Provided that $\norm{M^{-1/2} \Delta M^{-1/2}}_{op} < 1$ (which we will verify later), we have:
\begin{align*}
   X &= \calA^* \left( (\calA \calA^*)^{-1} 1_n \right)\\
   &= \calA^* \left( (M-\Delta)^{-1} 1_n \right) \\
   &= \calA^* \left( M^{-1/2}(I- M^{-1/2}\Delta M^{-1/2})^{-1} M^{-1/2} 1_n \right)\\
   &= \frac{1}{d(d-1)}\left(1-\frac{n}{n+d-1} \right)^{1/2} \calA^* \left( M^{-1/2} (I- M^{-1/2}\Delta M^{-1/2})^{-1} 1_n \right) \\
   &= \frac{1}{d(d-1)}\left(1-\frac{n}{n+d-1} \right)^{1/2} \calA^* \left( M^{-1/2} \left(I + M^{-1/2}\Delta M^{-1/2} + \sum_{j=2}^\infty (M^{-1/2}\Delta M^{-1/2})^j \right) 1_n \right)\\
   &\succeq \frac{1}{d(d-1)} \Bigg( \left(1-\frac{n}{n+d-1} \right) \lambda_{min} (\calA^* (1_n)) - \left(1-\frac{n}{n+d-1} \right) \norm{\calA^* \left(M^{-1} \Delta 1_n \right)}_{op} \\
   &\qquad- \left(1-\frac{n}{n+d-1} \right)^{1/2} \norm{\calA^* \left(M^{-1/2}\sum_{j=2}^\infty (M^{-1/2}\Delta M^{-1/2})^j 1_n \right)}_{op} \Bigg)I_d.
\end{align*}

{ \pax{
I got confused reading the previous display. There seem to be some incorrect factors of $1/d(d-1)$. Does below look correct?

First, I calculated
\[
M^{-1/2} 1_n = \frac{1}{\sqrt{d(n + d -1)} } 
= \frac{1}{\sqrt{d(d-1)}} ( 1 - \frac{n}{n + d -1} )^{1/2}. 
\]
Then I obtained
\begin{align*}
   X &= \calA^* \left( (\calA \calA^*)^{-1} 1_n \right)\\
   &= \calA^* \left( (M-\Delta)^{-1} 1_n \right) \\
   &= \calA^* \left( M^{-1/2}(I- M^{-1/2}\Delta M^{-1/2})^{-1} M^{-1/2} 1_n \right)\\
   &= \frac{1}{\sqrt{d(d-1)}}\left(1-\frac{n}{n+d-1} \right)^{1/2} \calA^* \left( M^{-1/2} (I- M^{-1/2}\Delta M^{-1/2})^{-1} 1_n \right) \\
   &= \frac{1}{\sqrt{d(d-1)}}\left(1-\frac{n}{n+d-1} \right)^{1/2} \calA^* \left( M^{-1/2} \left(I + M^{-1/2}\Delta M^{-1/2} + \sum_{j=2}^\infty (M^{-1/2}\Delta M^{-1/2})^j \right) 1_n \right)\\
   &\succeq \frac{1}{d(d-1)} \Bigg( \left(1-\frac{n}{n+d-1} \right) \lambda_{min} (\calA^* (1_n)) - \left(1-\frac{n}{n+d-1} \right) \norm{\calA^* \left(M^{-1} \Delta 1_n \right)}_{op} \\
   &\qquad- {\color{blue} \sqrt{d (d - 1)} } \left(1-\frac{n}{n+d-1} \right)^{1/2} \norm{\calA^* \bigg(M^{-1/2}\sum_{j=2}^\infty (M^{-1/2}\Delta M^{-1/2})^j 1_n \bigg)}_{op} \Bigg).
\end{align*}

In particular, I am concerned about the factor in blue because it will change the third bullet point below to something like:
\[
\norm{\calA^* M^{-1/2}\sum_{j=2}^\infty (M^{-1/2}\Delta M^{-1/2})^j 1_n}_{op} \ll \frac{1}{\sqrt{d(d-1)}}\left(1-\frac{n}{n+d-1} \right)^{1/2} \frac{c_0}{2}n
\ll \sqrt{\frac{n}{d}}. 
\]

% I can only show the previuos display holds whe

% I can only show the previous display holds when $n \ll d^{5/2}$: (which seems weird...)
% \begin{align*}
%     \norm{\calA^* \left(M^{-1/2} \sum_{j=2}^\infty (M^{-1/2}\Delta M^{-1/2})^j 1_n \right)}_{op} &\leq \norm{\calA^*}_{2 \rightarrow op} \norm{M^{-1/2} \sum_{j=2}^\infty (M^{-1/2}\Delta M^{-1/2})^j 1_n}_2 \\
%     &\leq \norm{\calA^*}_{2 \rightarrow op} \norm{M^{-1/2}}_{op} \norm{\sum_{j=1}^\infty (M^{-1/2}\Delta M^{-1/2})^j1_n}_{2} \\
%     &\leq (d + \sqrt{n}) \cdot \frac{1}{d} 
%      \cdot 
%     \| \sum_{j=2}^\infty (M^{-1/2}\Delta M^{-1/2})^j \|_{op} 
%     \cdot \frac{1}{\sqrt{nd}} \| M^{-1/2} \Delta  1_n \|_2 \\
%     &\leq (\frac{\sqrt{n}}{d})^2 \cdot \frac{1}{\sqrt{nd}} \cdot \frac{1}{d} 
%     \cdot n \sqrt{d} = 
%     \frac{n^{3/2}}{d^3}. 
% \end{align*}
% And
% \[
% \frac{n^{3/2}}{d^3} \leq \frac{n^{1/2}}{d^{1/2}} \Longleftrightarrow
% n \leq d^{5/2}. 
% \]
}
}


Observe that $\calA^* (1_n) = \sum_{i=1}^n v_i v_i^T$, so it follows from Theorem 4.7.1 of \cite{vershynin2018high} that with high probability $\lambda_{min} (\calA^* 1_n) \geq c_0 n$, for some positive constant $c_0$. To complete the proof, it suffices to verify that the following events hold with high probability:
\begin{itemize}
    \item $\norm{M^{-1/2} \Delta M^{-1/2}}_{op} < 1$,
    \item $\norm{\calA^* M^{-1} \Delta 1_n}_{op} \leq \frac{c_0}{2}n$,
    \item $\norm{\calA^* M^{-1/2}\sum_{j=2}^\infty (M^{-1/2}\Delta M^{-1/2})^j 1_n}_{op} \leq \left(1-\frac{n}{n+d-1} \right)^{1/2} \frac{c_0}{2}n$.
\end{itemize}
By Proposition~\ref{prop:delta-norm}, the first condition holds with high probability provided $n = o(d^2/\log^3 (d))$. For the second condition, note that 
\begin{align*}
    \norm{\calA^* \left( M^{-1} \Delta 1_n \right)}_{op} &\leq \norm{\calA^*}_{\infty \rightarrow op} \norm{M^{-1} \Delta 1_n}_{\infty} \\
    &\leq \norm{\calA^*}_{\infty \rightarrow op} \norm{M^{-1}}_{\infty \rightarrow \infty} \norm{\Delta 1_n}_{\infty}.
\end{align*}
With high probability, the first term is $\Theta(n)$ (by Lemma 2 of \cite{saunderson2012diagonal}), the second term is $\Theta (d^{-2})$ and the third term is $O(d \sqrt{n \log n})$ (by Proposition~\ref{prop:delta-ones-vector}), so their product is $o(n)$. For the third condition, we have
\begin{align*}
    \norm{\calA^* \left(M^{-1/2} \sum_{j=2}^\infty (M^{-1/2}\Delta M^{-1/2})^j 1_n \right)}_{op} &\leq \norm{\calA^*}_{2 \rightarrow op} \norm{M^{-1/2} \sum_{j=2}^\infty (M^{-1/2}\Delta M^{-1/2})^j 1_n}_2 \\
    &\leq \norm{\calA^*}_{2 \rightarrow op} \norm{M^{-1/2}}_{op} \norm{\sum_{j=1}^\infty (M^{-1/2}\Delta)^j M^{-1/2}}_{op} \\
    &\qquad\times \norm{M^{-1/2}\Delta M^{-1/2} 1_n}_2 \\
    &\leq \sqrt{n} \norm{\calA^*}_{2 \rightarrow op} \norm{M^{-1/2}}_{op} \norm{\sum_{j=1}^\infty (M^{-1/2}\Delta M^{-1/2})^j}_{op} \\
    &\qquad\times \norm{M^{-1/2}\Delta M^{-1/2} 1_n}_\infty \\
    &\leq \sqrt{n} \norm{\calA^*}_{2 \rightarrow op} \norm{M^{-1/2}}_{op} \sum_{j=1}^\infty \norm{(M^{-1/2}\Delta M^{-1/2})}^j_{op} \\
    &\qquad\times \norm{M^{-1/2}}_{\infty \rightarrow \infty} \norm{\Delta M^{-1/2} 1_n}_\infty \\
    &= \left(\frac{1}{d(n+d-1)} \right)^{1/2} \sqrt{n} \norm{\calA^*}_{2 \rightarrow op} \norm{M^{-1/2}}_{op} \\
    &\qquad\times \frac{\norm{M^{-1/2}\Delta M^{-1/2}}_{op}}{1- \norm{M^{-1/2}\Delta M^{-1/2}}_{op}} \norm{M^{-1/2}}_{\infty \rightarrow \infty} \norm{\Delta 1_n}_\infty \\
    &\leq \left(\frac{1}{d(n+d-1)} \right)^{1/2} \sqrt{n} \times \Theta(d + \sqrt{n}) \times \frac{1}{\sqrt{d^2 - d}} \\
    &\qquad\times o(1) \times O(1) \times O(d\sqrt{n \log n}),
\end{align*}



where the last step holds with high probability since with high probability $\norm{\calA^*}_{2 \rightarrow op} = \Theta(d + \sqrt{n})$ (by Lemma 3 of \cite{saunderson2011subspace}), $\norm{M^{-1/2}\Delta M^{-1/2}}_{op} = o(1)$ (by Proposition~\ref{prop:delta-norm}), $\norm{\Delta 1_n}_\infty = O(d\sqrt{n \log n})$ (by Proposition~\ref{prop:delta-ones-vector}) and $\norm{M^{-1/2}}_{op} = (d^2-d)^{-1/2}, \norm{M^{-1/2}}_{\infty \rightarrow \infty} = O(1)$. Altogether, these bounds suffice to show the third condition is satisfied with high probability for some $n = \Omega(d/ \log^5 (d))$.
\end{proof}


\section{Proof of Proposition~\ref{prop:delta-norm}}
\label{sec:convergence-criterion}
The goal of this section is to upper bound the quantity $\norm{M^{-1/2} \Delta M^{-1/2}}_{op}$. The proof of Proposition~\ref{prop:delta-norm} relies on the supporting Lemmas \ref{lemma:weak-delta-bound} and \ref{lem:delta-ones-perp} below that are later proved in Section \ref{subsec:supporting_lemmas}. The first lemma prescribes a rough bound on
\begin{align*}
    \norm{\Delta}_{op} = 
\sup_{u \,:\, \| u \|_2 = 1}     \big| u^T \Delta u  \big|,
\end{align*} 
and the second gives a sharper bound on the above quadratic form when restricting to vectors orthogonal to $1_n$. 
\begin{lemma}
\label{lemma:weak-delta-bound}
With high probability, $\norm{\Delta}_{op} = O(n \sqrt{d} \log^2 (n) + d \sqrt{n} \log^4 (dn))$.
\end{lemma}

\begin{lemma}
\label{lem:delta-ones-perp}
With high probability,
\[
\sup_{\norm{u}_2 =1,\, u \perp 1_n} |u^T \Delta u| = O(n \log^3 (dn) + d \sqrt{n} \log^4 (dn)).
\]
\end{lemma}


\begin{proof}[Proof of Proposition~\ref{prop:delta-norm}]
We upper bound the quantity $|u^T M^{-1/2} \Delta M^{-1/2} u|$ uniformly over all $u \in \R^n$ with $\norm{u}_2 = 1$. We decompose $u = \ip{u}{\frac{1}{\sqrt{n}}1_n} \frac{1}{\sqrt{n}}1_n + u^{\perp}$, where $u^\perp$ satisfies $\ip{u^\perp}{1_n} = 0$. Plugging in this decomposition and expanding, we have:
\begin{align*}
u^T M^{-1/2} \Delta M^{-1/2}u &= \ip{u}{\frac{1}{\sqrt{n}}1_n}^2 \frac{1}{\sqrt{n}}1_n^T M^{-1/2} \Delta M^{-1/2} \frac{1}{\sqrt{n}}1_n + \ip{u}{\frac{1}{\sqrt{n}}1_n} u^{\perp T} M^{-1/2} \Delta M^{-1/2} \frac{1}{\sqrt{n}}1_n \\
&\qquad+ u^{\perp T} M^{-1/2} \Delta M^{-1/2} u^{\perp} + \ip{u}{\frac{1}{\sqrt{n}}1_n} \frac{1}{\sqrt{n}} 1_n^T M^{-1/2} \Delta M^{-1/2} u^\perp \\
&= \ip{u}{\frac{1}{\sqrt{n}}1_n}^2 \frac{1}{dn(n+d-1)} 1_n^T \Delta 1_n + \frac{\ip{u}{\frac{1}{\sqrt{n}}1_n}}{\sqrt{d^2 - d}}  \frac{1}{\sqrt{dn(n+d-1)}} u^{\perp T} \Delta 1_n \\
&\qquad+ \frac{1}{d^2 - d} u^{\perp T} \Delta u^{\perp} + \frac{\ip{u}{\frac{1}{\sqrt{n}}1_n}}{\sqrt{d^2 - d}} \frac{1}{\sqrt{dn(n+d-1)}} 1_n^T \Delta u^{\perp}.
\end{align*}
We proceed to upper bound the absolute value of each of these four terms. For the first term, we have
\begin{align*}
\ip{u}{\frac{1}{\sqrt{n}}1_n}^2 \frac{1}{dn(n+d-1)} |1_n^T \Delta 1_n| &\leq  \frac{1}{dn(n+d-1)} |1_n^T \Delta 1_n| \\
&\leq \frac{1}{dn(n+d-1)} \norm{1_n}_2 \norm{\Delta 1_n}_2 \\
&\leq \frac{1}{d(n+d-1)} \norm{\Delta 1_n}_\infty.
\end{align*}
With high probability, for any $u$, the first term is $O(\sqrt{\log(n) / n} + \log(n) / \sqrt{dn})$ (by Proposition~\ref{prop:delta-ones-vector}). Next, note that the second and fourth terms are equal by symmetry of $\Delta$. We can bound the absolute value of the fourth term as follows:
\begin{align*}
\frac{\left| \ip{u}{\frac{1}{\sqrt{n}}1_n} \right|}{\sqrt{d^2 - d}} \frac{1}{\sqrt{d n(n+d-1)}}  |1_n^T \Delta u^{\perp}| &\leq \frac{1}{\sqrt{d^2 - d}} \frac{1}{\sqrt{dn(n+d-1)}} \norm{1_n}_2 \norm{\Delta u^{\perp}}_2 \\
&\leq \frac{1}{\sqrt{d^2 - d}} \frac{1}{\sqrt{d(n+d-1)}} \norm{\Delta}_{op}. 
\end{align*}
By Lemma~\ref{lemma:weak-delta-bound}, with high probability, for any $u$, the second and fourth terms are $O(\sqrt{n} \log^2 (n)/d)$. Applying Lemma~\ref{lem:delta-ones-perp} to upper bound the absolute value of the third term and summing the bounds for each of the four terms completes the proof.
\end{proof}

\subsection{Supporting lemmas for Proposition~\ref{prop:delta-norm}}
\label{subsec:supporting_lemmas}
The proofs of Lemmas \ref{lemma:weak-delta-bound}
and \ref{lem:delta-ones-perp} rely on the following useful decomposition of $\calA \calA^*$. First, for every $i \in [n]$, define $u_i = v_i \otimes v_i \in \R^{d \times d}$, $\offdiag (u_i)$ to be the flattening of the (non-diagonal) upper triangle of entries of $u_i$ as a vector in $\R^{d(d-1)/2}$, and $\diag (u_i)$ to be the flattening of the diagonal of $u_i$ as a vector in $\R^d$. Next, define $U_{\offdiag} \in \R^{(d(d-1)/2) \times n}$ and $U_{\diag} \in \R^{d \times n}$ to be the matrices whose $i^{\text{th}}$ columns are $\offdiag(u_i)$ and $\diag(u_i)$, respectively. With this notation in hand, we can express $\calA \calA^* = U_{\diag}^T U_{\diag} + 2U_{\offdiag}^T U_{\offdiag}$ as the sum of two Gram matrices and $\Delta = \Delta' + \Delta''$, where $\Delta' = d 1_n 1_n^T - U^T_{\diag} U_{\diag}$ and $\Delta'' = (d^2-d) I_n - 2 U^T_{\offdiag} U_{\offdiag}$. 

In the following, we will show that the dominant contribution to $\norm{\Delta}_{op}$ comes from $\Delta'$ (corresponding to deviations along the $1_n$ direction) and $\Delta''$ essentially behaves like a Wishart matrix with significantly smaller norm. The above decomposition of $\Delta$ allows us to ``separate''  large quadratic forms of $M^{-1/2} \Delta M^{-1/2}$ into two cases, corresponding to vectors aligned with and othogonal to $1_n$, and analyze each using different arguments. 

\subsubsection{Proof of Lemma~\ref{lemma:weak-delta-bound}}
The goal of this section is to bound $\norm{\Delta}_{op}$. The proof of Lemma~\ref{lemma:weak-delta-bound} follows immediately from the following two lemmas and an application of Markov's inequality.

\begin{lemma}
\label{lemma:delta-prime}
With high probability, $\norm{\Delta'}_{op} = O(d + n \sqrt{d}  \log^2 (n))$.
\end{lemma}


\begin{lemma}
\label{lemma:delta-double-prime}
$\E \norm{\Delta''}_{op} = O(d \sqrt{n} \log^3 (dn) + n)$.
\end{lemma}


\begin{proof}[Proof of Lemma~\ref{lemma:delta-prime}]
First, note that
\[
\norm{\Delta'}_{op} \leq \norm{d 1_n 1_n^T - \E U^T_{\diag} U_{\diag}}_{op} + \norm{\E U^T_{\diag} U_{\diag} - U^T_{\diag} U_{\diag}}_{op} = \norm{2d I_n}_{op} + \norm{\E U^T_{\diag} U_{\diag} - U^T_{\diag} U_{\diag}}_{op}.
\]
To control the second term, note that the $(i,j)$ entry of $U^T_{\diag} U_{\diag} - \E U^T_{\diag} U_{\diag}$ is the sum of $d$ independent random variables which are mean-zero, constant variance and a product of a pair of subexponential random variables:
\[
(U^T_{\diag} U_{\diag} - \E U^T_{\diag} U_{\diag})_{ij} = \sum_{k=1}^d (v_i)_k^2 (v_j)_k^2 - (1 + 2 \I \{i=j\}).
\]
By Theorem~\ref{thm:gaussian-poly-conc}, each entry $e$ admits a tail-bound of the form:
\[
\Prob (|e| > t \sqrt{d}) \leq \exp \left(-C \cdot\sqrt{t} \right),
\]
for some constant $C$. Taking $t = O(\log^2 (n))$ large enough and applying a union bound over all $n^2$ entries, we may conclude that with probability $1-o(1)$, all entries of $U^T_{\diag} U_{\diag} - \E U^T_{\diag} U_{\diag}$ are bounded by $t$ in absolute value. In particular, every row has norm at most $O(\sqrt{nd} \log(n))$ . Since the operator norm is at most $\sqrt{n}$ times the maximum row norm, we may conclude $\norm{\Delta'}_{op} = O(n \sqrt{d} \log (n))$.
\end{proof}

%Another way  to bound $\norm{\Delta'}$ is to use a truncated matrix Bernstein inequality (see Proposition A.7 of \cite{hopkins2015fast}).


\begin{proof}[Proof of Lemma~\ref{lemma:delta-double-prime}]
We make use of a variant of Theorem 5.62 of \cite{vershynin2010introduction}, see Theorem~\ref{thm:vershynin-562}. To apply this theorem, we must verify that the columns of $U_{\offdiag}$ are independent and isotropic random vectors. First, the columns of $U_{\offdiag}$ are independent because column $i$ depends only on $v_i$. To verify isotropy, note that since the columns are identically distributed, it suffices to verify it for the first column $\offdiag(u_1)$. The $(i,j)$ coordinate (for $i,j \in [d]$ and $i < j$) is $(v_1)_i (v_1)_j$, which has mean zero, since $i \neq j$. The $((i,j), (k,l))$ (again, for $i,j,k, l \in [d]$ and $i < j$ and $k < l$) entry of the covariance matrix of $\offdiag(u_1)$ is $\E (v_1)_i (v_1)_j (v_1)_k (v_1)_l = \I \{(i,j) = (k,l)\}$. We may conclude that the columns are indeed isotropic.

Letting $N = \frac{(d^2 -d)}{2}$ and applying Theorem~\ref{thm:vershynin-562} yields, for some constant $C > 0$,
\[
\E \norm{U_{\offdiag}^T U_{\offdiag} - N I_n}_{op} \leq C \left( \sqrt{N m \log n} + \sqrt{N n \log n} \cdot \E \max_{i \in [n]} \sqrt{1 + \epsilon_i} + N \cdot \E \max_{i \in [n]} | \epsilon_i | \right)
\]
where 
\[
m = \frac{1}{N} \E \max_{j \leq n} \sum_{k \neq j}  \ip{\offdiag(u_j)}{\offdiag(u_k)}^2,
\]
and
\[
\epsilon_i = \frac{1}{N} \norm{\offdiag(u_i)}^2_2 - 1.
\]
The following two claims, whose proofs we defer to Appendix~\ref{sec:technical-lemmas}, give upper bounds on the parameters $m$ and $\epsilon_i$.
\begin{claim}
\label{claim:m-parameter-bound}
$m = O(n \log^5 (dn))$.
\end{claim}


\begin{claim}
\label{claim:eps-bound}
$\E \max_{i \in [n]} | \epsilon_i | = O\left(\frac{\log d}{\sqrt{d}} + \frac{n}{N}\right)$.
\end{claim}
Applying Claims~\ref{claim:m-parameter-bound} and \ref{claim:eps-bound} and the fact that 
\[
\E \max_{i \in [n]} \sqrt{1 + \epsilon_i} \leq \E \max_{i \in [n]} \sqrt{1 + |\epsilon_i|} \leq  \E \max_{i \in [n]} \sqrt{1} + \sqrt{|\epsilon_i|} \leq 1 + \sqrt{\E \max_{i \in [n]} |\epsilon_i|},
\]
we conclude:
\[
\E \norm{2 U_{\offdiag}^T U_{\offdiag} - (d^2 - d) I_n}_{op}  = O(d \sqrt{n} \log^3 (dn) + n). \qedhere
\]
\end{proof}


\subsubsection{Proof of Lemma~\ref{lem:delta-ones-perp}}
Now, we turn our attention to controlling the restricted supremum $\sup_{\norm{u}_2 =1, u \perp 1_n} |u^T \Delta u|$. First, recall the decomposition $\Delta = \Delta' + \Delta''$ and that we have already shown $\E \norm{\Delta''}_{op} = O(d \sqrt{n} \log^3 (dn) + n)$ in Lemma~\ref{lemma:delta-double-prime}. To complete the proof, we show, by a union bound, that 
\[
\sup_{\norm{u}_2 =1,\, u \perp 1_n} |u^T \Delta' u| \lesssim n \log^3 (dn)
\]
with high probability. 

Set $\epsilon = d^{-1/2}$ and let $\calN_0$ be an $\epsilon$-net of the unit sphere in $\R^n$. By Corollary 4.2.13 of \cite{vershynin2018high}, there exists such an $\calN_0$ of size $|\calN_0| \leq (1 + \frac{2}{\epsilon})^n$. Next, define $\Pi$ to be the projection onto the subspace of vectors orthogonal to $1_n$ and $\calN_1 = \{\Pi u : u \in \calN_0\}$. Note that since $\norm{\Pi u - \Pi v}_2 \leq \norm{u-v}_2$, it holds that $\calN_1$ is an $\epsilon$-net for the set $S = \{u \in \R^n: \norm{u}_2 = 1, u \perp 1_n\}$. For every vector $u \in S$ we may write $u = \hat{u} + \delta_u$, where $\hat{u}$ is in $\calN_1$ and $\norm{\delta_u}_2 \leq \epsilon$. We now have the following:
\begin{align*}
\sup_{\norm{u}_2 =1,\, u \perp 1_n} |u^T \Delta' u| &\leq  \max_{\hat{u} \in \calN_1} |\hat{u}^T \Delta' \hat{u}| + \sup_{\norm{u}_2 =1,\, u \perp 1_n} |\hat{u}^T \Delta' \delta_u| \\
&+ \sup_{\norm{u}_2 =1,\, u \perp 1_n} |\delta_u \Delta' \hat{u}| + \sup_{\norm{u}_2 =1,\, u \perp 1_n} |\delta_u \Delta' \delta_u| \\
&\leq \sup_{\hat{u} \in \calN_1} |\hat{u}^T \Delta' \hat{u}| + \epsilon \norm{\Delta'}_{op} \\
&+ \epsilon \norm{\Delta'}_{op} + \epsilon^2 \norm{\Delta'}_{op}.
\end{align*}
By Lemma~\ref{lemma:delta-prime} and our choice of $\epsilon = d^{-1/2}$, the last three terms are $O(\sqrt{d} + n \log^2 (n))$ with high probability. 

To control the first term, we begin by introducing some notation. Let $s_1, \ldots, s_n \sim (\chi_1^2)^{\otimes d}$ and for every $u \in \R^n$, define $\sigma (u) = \sum_{i=1}^n u_i s_i$. Note that the collection of random variables $\{\Delta'_{ij}: i,j \in [n]\}$ has the same joint distribution as $\{(\E \ip{s_i}{s_j}) - \ip{s_i}{s_j}: i,j \in [n]\}$. Hence, for any fixed $u \in \R^n$ we have that $u^T \Delta' u$ has the same distribution as $\norm{\sigma (u)}_2^2 - \E \norm{\sigma (u)}_2^2$. Now, define $E$ to be the event that $|(s_i)_j| \leq B$ for all $i \in [n], j \in [d]$ and some $B = O(\log (dn))$ sufficiently large. Finally, define $\E (\norm{\sigma (u)}_2^2 \mid E)$ to be the expectation of the random variable $\norm{\sigma (u)}_2^2$ conditioned on the event $E$ and let $t > 0$ be a parameter to be determined later. Given this, we have that
\begin{align*}
\Prob \left( \max_{u \in \calN_1} |u^T \Delta' u| \leq t \right) &= \Prob \left( \max_{u \in \calN_1} |\norm{\sigma (u)}_2^2 - \E \norm{\sigma (u)}_2^2| \leq t \right) \\
&\geq \Prob \left( E \wedge \max_{u \in \calN_1} |\norm{\sigma (u)}_2^2 - \E \norm{\sigma (u)}_2^2| \leq t \right) \\ 
&= \Prob(E) \Prob \left(\max_{u \in \calN_1} |\norm{\sigma (u)}_2^2 - \E \norm{\sigma (u)}_2^2| \leq t \;\middle|\; E \right) \\
&= \Prob(E) \left( 1- \Prob \left(\max_{u \in \calN_1} |\norm{\sigma (u)}_2^2 - \E \norm{\sigma (u)}_2^2| > t \;\middle|\; E \right) \right) \\
&\geq \Prob(E) \left( 1- |\calN_1| \max_{u \in \calN_1} \Prob \left( |\norm{\sigma (u)}_2^2 - \E \norm{\sigma (u)}_2^2| > t \;\middle|\; E \right) \right).
\end{align*}
By a straightforward application of the union bound and a tail bound for the $\chi_1^2$ distribution, it follows that $\Prob (E) \geq 1-o(1)$ for some $B = O(\log (dn))$. We now complete the proof by showing that there is a choice of $t = O(n \log^3 (dn))$ such that for any $u \in \calN_1$, it holds that $\Prob \left( |\norm{\sigma (u)}_2^2 - \E \norm{\sigma (u)}_2^2| > t \;\middle|\; E \right) = o(\sqrt{d}^{-n})$.

Since we are conditioning on the event $E$, we need to re-center the random variable $\norm{\sigma (u)}_2^2$. We bound the difference in expectations before and after conditioning in the following way, for every $u \in \calN_1$:
\begin{align*}
|\E (\norm{\sigma (u)}_2^2 \mid E) - \E \norm{\sigma (u)}_2^2 | &\leq d |\E \sigma(u)_1^2 - \E (\sigma(u)_1^2 \mid E)| \\
&\leq d \left( |\Var (\sigma(u)_1) - \Var (\sigma(u)_1 \mid E)| + |(\E \sigma(u)_1)^2 - (\E (\sigma(u)_1 \mid E))^2| \right) \\
&= d \left( \left| \sum_{i=1}^n u_i^2 (\Var((s_i)_1) - \Var((s_i)_1 \mid E)) \right| + |(\E \sigma(u)_1)^2 - (\E (\sigma(u)_1 \mid E))^2|\right) \\
&\leq d \left( 2 \norm{u}_2^2 + |(\E \sigma(u)_1)^2 - (\E (\sigma(u)_1 \mid E))^2|\right) \\
&= d \left( 2 \norm{u}_2^2 + |(\ip{u}{1_n}^2 - \ip{u}{1_n}^2 (\E ((s_1)_1 \mid E))^2|\right) \\
&= d (2 \norm{u}_2^2 + \ip{u}{1_n}^2 (1- (\E ((s_1)_1 \mid E))^2)) \leq 2d
\end{align*}
where in the third inequality we used the fact that the conditional $\chi^2_1$ distribution only has a smaller variance and in the last step we used the facts that $\norm{u}_2^2 \leq 1$ and $\ip{u}{1_n} = 0$. Applying the triangle inequality then yields
\[
\Prob \left( |\norm{\sigma (u)}_2^2 - \E \norm{\sigma (u)}_2^2| > t \;\middle|\; E \right) \leq \Prob \left( |\norm{\sigma (u)}_2^2 - \E (\norm{\sigma (u)}_2^2 \mid E)| > t -2d \;\middle|\; E \right).
\]

To upper bound the latter tail probability, note that (on the event $E$),
\[
\norm{\sigma (u)}_2^2 - \E (\norm{\sigma (u)}_2^2 \mid E) = \sum_{i=1}^d \sigma(u)_i^2 - \E (\sigma(u)_i^2 \mid E)
\]
is a sum of mean-zero i.i.d.\ random variables. We show that each $\sigma(u)_i$ is a sub-gaussian random variable with sub-gaussian parameter $O(B)$. Given this, we conclude that each $\sigma(u)_i^2 - \E (\sigma(u)_i^2 \mid E)$ is sub-exponential with parameter $O(B^2)$ (see Lemma 2.7.6 and Exercise 2.7.10 of \cite{vershynin2018high}). By Bernstein's inequality (see Theorem 2.8.1 of~\cite{vershynin2018high}), it holds that, for some constant $c > 0$ and any $s \geq 0$,
\[
\Prob \left(\left| \norm{\sigma (u)}_2^2 - \E (\norm{\sigma (u)}_2^2 \mid E) \right| > s \;\middle|\; E \right) \leq 2 \exp \left(-c \min \left( \frac{s^2}{dB^4}, \frac{s}{B^2}\right) \right).
\]
Setting $s = t - 2d$ and $t = O(n \log^3 (dn))$ large enough is sufficient to ensure that
\[
|\calN_1| \max_{u \in \calN_1} \Prob \left( |\norm{\sigma (u)}_2^2 - \E \norm{\sigma (u)}_2^2| > t \;\middle|\; E \right) \leq (1 + 2 \sqrt{d})^n \exp(-100 n \log (d))= o(1).
\]

Finally, we show that $\sigma(u)_1$ is a sub-gaussian random variable with parameter $O(B)$. Expanding the definition, we have
\[
\sigma(u)_1 = (\sigma(u)_1 - \E (\sigma(u)_1 \mid E)) + \E (\sigma(u)_1 \mid E) = \left( \sum_{i=1}^n u_i ((s_i)_1 - \E ((s_i)_1 \mid E)) \right) + \E ((s_1)_1 \mid E) \ip{u}{1_n}.
\]
Observe that since $(s_i)_1 \leq B$, the first summation of independent mean-zero sub-gaussian random variables is itself a sub-gaussian random variable with sub-gaussian parameter $O(B \cdot \norm{u}_2) = O(B)$ (see Proposition 2.6.1 of \cite{vershynin2010introduction}). Since $u \perp 1_n$, the second term is zero. We may conclude that $\sigma(u)_1$ is subgaussian with parameter $O(B)$.

\section{Proof of Proposition~\ref{prop:delta-ones-vector}}
\label{sec:delta-ones-vector}
To upper bound $\norm{\Delta 1_n}_{\infty}$, it suffices to prove a bound of the form
\[
\Prob (|(\Delta 1_n)_1| > t) = o(n^{-1}),
\]
so that we may union bound over the $n$ identically distributed coordinates. We have that
\[
(\Delta 1_n)_1 = (\E \ip{v_1}{v_1}^2) - \ip{v_1}{v_1}^2 + \sum_{i=2}^n (\E \ip{v_1}{v_i}^2) - \ip{v_1}{v_i}^2.
\]
The absolute value of the first difference is $O(d^{3/2} \log n)$ with probability $1- o(n^{-1})$. To see this, note that $\E \ip{v_1}{v_1}^2 = d^2 + 2d$ and $\ip{v_1}{v_1} \sim \chi^2_d$. By Bernstein's inequality (see Theorem 2.8.1 of \cite{vershynin2018high}), it holds that $\ip{v_1}{v_1} = d \pm O(\sqrt{d \log n})$ with probability $1- o(n^{-1})$. Squaring this expression out and taking the difference with $d^2 + 2d$ yields a bound of $O(d^{3/2} \log n)$.

For the remaining terms, observe that conditioned on $v_1$, each of $\ip{v_1}{v_i}$ is distributed as $\norm{v_1}_2 g_i$, where $g_i \sim \calN(0,1)$  (for $i > 1$). Conditioned on $v_1$, the remaining terms of the summation are distributed as 
\[
\norm{v_1}_2^2 \left((n-1) -  \sum_{i=2}^n g_i^2 \right).
\]
Again by Bernstein's inequality, since $\sum_{i=2}^n g_i^2 \sim \chi^2_{n-1}$, it holds that the absolute difference of this random variable and its mean $(n-1)$ is $O(\sqrt{n \log n})$ with probability $1- o(n^{-1})$. As before, $\norm{v_1}_2^2 = d \pm O(\sqrt{d \log n})$ with probability $1- o(n^{-1})$. Putting these bounds together concludes the proof.



==> Notes/graph_matrices_with_comments_Nov7_30minsbeforedeadline.tex <==

\section{Graph matrices}
\label{sec:graph_matrices}
\subsection{Background}

We use the theory of \textit{graph matrices} to derive operator norm bounds on various random matrices that arise in our analysis. For our setting, we can define graph matrices as follows. These definitions are a special case of the definitions in \cite{ahn2016graph} and are equivalent to the definitions in \cite{ghosh2020sum} except that instead of summing over ribbons, we sum over injective maps. This gives a constant factor difference (see Remark 2.17 of \cite{ahn2016graph}) in the final norm bounds.


In our analysis, many of the matrices we study, such as $\Delta^k$ are $n \times n$ and have entries that are sums of terms of the form
\begin{align}
\label{eqn:generic_term}
M_{i_1, i_r} = \sum_{\substack{i_2, \ldots, i_{r-1} \\ k_1, \ldots, k_s} }
\prod_{x = 1}^r \prod_{y = 1}^s 
f_{x, y}( v_{i_x, k_y} )
\end{align}
where $ v_{i_x, k_y}$ is the $k_y$ coordinate of $v_{i_x}$, $\{ f_{x, y}\}$ are low-degree Hermite polynomials, and the indices of summation obey certain restrictions. These restrictions imply for one that $i_2, \ldots, i_{r-1}$ are required to be distinct as well as $k_1, \ldots, k_{s}$.

The framework of graph matrices provides a convenient way of encoding these restrictions and attaining good norm bounds. Concretely, each matrix as in term \eqref{eqn:generic_term} can be represented by a `shape' consisting of a graph with $r$ circle vertices, $s$ square vertices, and integer edge labels. For a term like \eqref{eqn:generic_term} which is an $n \times n$ matrix, there are two distinguished circle vertices that represent $i_1$ and $i_r$. The edges in the shape designate terms in the product in \eqref{eqn:generic_term} that are nontrivial in that they are not equal to $1$, and the vertices specify (distinct) indices of summation. The remaining circle vertices each represent an index of summation over $1 \leq i \leq n$ (ie, one of $i_2, \ldots, i_r$) and a square vertex is used to represent an index of summation over $1 \leq k \leq d$ (ie, one of $k_1, \ldots, k_s$, each of which indexes the dimension). The integer edge labels of the shape denote the degree of the Hermite polynomial that is applied to the random variable $v_{i_x, k_y}$. We make this precise with the following definitions. 

As another preliminary we define the (normalized) Hermite polynomials

\begin{definition}[Normalized Hermite polynomials (see e.g. \cite{odonnell}, Chapter 11.2)]
\label{def:hermite} 
    Define the sequence of normalized Hermite polynomials $h_0, h_1, h_2,\ldots$ by
    \[
h_j  = \frac{1}{\sqrt{j!}} \cdot H_j,
    \]
    where $H_j$ are defined uniquely by the following formal power series in $z$: 
    \[
\exp( tz - \frac{1}{2} t^2)
=\sum_{j = 0}^\infty \frac{1}{j!} H_j(z) t^j. 
    \]
\end{definition}
The first few Hermite polynomials are
\[
h_0(z) = 1, 
h_1(z) = z, h_2(z) = \frac{1}{\sqrt{2}} (z^2 - 1), 
h_3(z) = \frac{z^3 - 3z}{\sqrt{6}}, \ldots 
\]
Recall $\E_{Z \sim N(0,1)}[ h_j(Z) h_k(Z)] = \delta_{jk}$, where $\delta_{jk}$ denotes the Kronecker function. 

\pax{The notation $\alpha$ is now overloaded to be the scalar $\approx d^2$ and also to stand for a shape. This might be fine though. }

\begin{definition}
A shape $\alpha$ consists of the following:
\begin{enumerate}
    \item A set of circle and square vertices $V(\alpha)$. We take $V_{\circ}(\alpha)$ to be the set of circle vertices in $V(\alpha)$ and we take $V_{\Box}(\alpha)$ to be the set of square vertices in $V(\alpha)$.


    
    \item Distinguished tuples of vertices $U_{\alpha}$ and $V_{\alpha}$ (which may intersect) which we call the left and right sides of $\alpha$. We take $U_{\alpha,\circ}$ to be the circle vertices of $U_{\alpha}$ (in the same order) and we take $U_{\alpha,\Box}$ to be the square vertices of $U_{\alpha}$ (in the same order). Similarly, we take $V_{\alpha,\circ}$ to be the circle vertices of $V_{\alpha}$ (in the same order) and we take $V_{\alpha,\Box}$ to be the square vertices of $V_{\alpha}$ (in the same order).

\pax{I find it syntactically  very confusing that $V(\alpha)$ and $V_\alpha$ have such different meanings. What if we use a different font like $\mathcal{V}(\alpha)$ to denote the vertices in the shape $\alpha$?} \aw{agreed} \pax{Okay, let's make this change thorughout when rest of proof is solidified.}
    
    \item A set $E(\alpha)$ of edges where each edge is between a circle vertex and a square vertex. For each edge $e \in E(\alpha)$, we have a label $l_e \in \mathbb{N}$. We define $|E(\alpha)|$ to be $|E(\alpha)| = \sum_{e \in E(\alpha)}{l_e}$. \aw{does $\mathbb{N}$ include $0$? I think we should not allow $0$ as a label (should just be a non-edge)?}
\end{enumerate}
\end{definition}



Add explanation here.
\begin{definition}
\label{def:graph_matrix}
Given a shape $\alpha$, we define $M_{\alpha}$ to be the $\frac{n!d!}{(n- |U_{\alpha,\circ}|)!(d- |U_{\alpha,\Box}|)!} \times \frac{n!d!}{(n- |V_{\alpha,\circ}|)!(d- |V_{\alpha,\Box}|)!}$ matrix with entries
\[
M_{\alpha}(A,B) = \sum_{{{\pi_{\circ}: V_{\circ}(\alpha) \to [n], \pi_{\Box}: V_{\Box}(\alpha) \to [d]: \atop 
\pi_{\circ}, \pi_{\Box} \text{ are injective}} \atop 
\pi_{\circ}(U_{\alpha,\circ}) = A_{\circ}, \pi_{\Box}(U_{\alpha,\Box}) = A_{\Box},} \atop 
\pi_{\circ}(V_{\alpha,\circ}) = B_{\circ}, \pi_{\Box}(V_{\alpha,\Box}) = B_{\Box}}{\left(\prod_{e = \{u,v\} \in E(\alpha): u \in V_{\circ}(\alpha), y \in V_{\Box}(\alpha)}{h_{l_e}(v_{\pi_{\circ}(u), \pi_{\Box}(y)})}\right)}.
\]
where $A = ( A_{\circ}, A_{\Box})$ is an ordered tuple such that $A_{\circ}$ is an ordered tuple of $|U_{\alpha,\circ}|$ elements from $[n]$ and $A_{\Box}$ is an ordered tuple of $|U_{\alpha,\Box}|$ elements from $[d]$; and $B = ( B_{\circ}, B_{\Box})$ is an ordered tuple such that $B_{\circ}$ is an ordered tuple of $|V_{\alpha,\circ}|$ elements from $[n]$ and $B_{\Box})$ is an ordered tuple of $|V_{\alpha,\Box}|$ elements from $[d]$. 
  % $A_{\circ}$ consists of the elements $A$ (in the same order), $A_{\Box}$ consists of the square vertices of $A$ (in the same order), $B_{\circ}$ consists of the circle vertices of $B$ (in the same order), and $B_{\Box}$ consists of the square vertices of $B$ (in the same order).
\end{definition}

The proofs of Lemmas~\ref{lemma:Astar-Binv-1} and~\ref{lemma:Astar-Binv-w} boil down to obtaining norm bounds on $\calA^* (\Delta^k z)$ for $z \in \{1_n, w\}$. Such a matrix is $ d \times d$ and can be expressed as a sum of terms that are similar to \eqref{eqn:generic_term}:
\begin{align}
M_{k_1, k_s} = \sum_{\substack{i_1,i_2, \ldots, i_{r-1}, i_r \\ k_2, \ldots, k_{s-1}} }
\prod_{x = 1}^r \prod_{y = 1}^s 
f_{x, y}( v_{i_x, k_y} )
\end{align} 
where again this is a graph matrix, and restrictions on the indices are encoded by an associated shape as described in Definition~\ref{def:graph_matrix}. The difference between this and \eqref{eqn:generic_term} is that the distinguished vertices are now both squares instead of circles. Also note that the restrictions imply that $i_1, \ldots, i_r$ are distinct as well as $k_2, \ldots, k_{s-1}$.

\TODO{Add explanation and examples here.}


As mentioned, graph matrices have good norm bounds provided by the next result that follows from \cite{ahn2016graph}. Its proof is postponed to Appendix \ref{sec:norm_bounds}. 

To state the theorem below, we borrow some notions from \cite{ahn2016graph}. Given a shape $\alpha$ and a vertex $a \in \alpha$, we define 
\[
\varphi(a) =\begin{cases}
1 \quad &\text{if } a \text{ is a circle} \\
\log_n(d) \quad &\text{if } a \text{ is a square}
\end{cases} 
\]
Given a (potentially empty) subset of vertices $S \subset \alpha$, define $\varphi(S) = \sum_{s \in S} \varphi(s)$. Define the \textit{min-vertex separator} $S_{\min}$ of $\alpha$ to be a (potentially empty) subset of  vertices of $ \alpha$ with the smallest value of $\varphi(S)$ such that all paths from $U_\alpha$ to $V_\alpha$ intersect $S$. Here we allow for paths of length $0$, so any separator between $U_\alpha$ and $V_\alpha$ must contain $U_\alpha \cap V_\alpha$. 
% if $a$ and its incident edges are removed from $\alpha$. 
We also define $Iso(\alpha)$ to consist of all isolated vertices lying in $V(\alpha)\backslash ( U_\alpha \cup V_\alpha)$. 

\begin{theorem}[Theorem \ref{thm:graph-matrix-norm-bound}]
\label{thm:graph-matrix-norm-bound}
	Given $D_V,D_E \in \mathbb{N}$ such that $D_E \geq D_V \geq 2$ and $\epsilon > 0$, with probability at least $1 - \epsilon$, for all shapes $\alpha$ on square and circle vertices such that $|V(\alpha)| \leq D_V$, $|E_{\alpha}| \leq D_E$, and $U_{\alpha}$ and $V_{\alpha}$ either both contain one circle vertex or both contain one square vertex (which may be the same vertex), \[
	\|M_{\alpha}\|_{op} \leq \left((2D_E + 2)ln(D_V) + ln(4n) + ln\left(\frac{1}{\epsilon}\right)\right)^{|V(\alpha)| + |E(\alpha)|}n^{\frac{\varphi(V(\alpha)) - \varphi(S_{min}) + \varphi(Iso(\alpha))}{2}}
	\]
	where $S_{min}$ is a min-vertex separator of $\alpha$.
 \pax{Trying to avoid overusing the term `weight' here... please check if clear }
\end{theorem}

In our applications of this result, we invoke this result with $\epsilon = 1/poly(n)$ on shapes $\alpha$ for which $|V(\alpha)|, |E_\alpha
| \leq O(\polylog(n))$,so that the norm bounds take the form L
\[
\| M_\alpha \|_{op} = (\polylog(n))^{O(|V(\alpha)| + |E(\alpha)|)} \cdot n^{\frac{\varphi(V(\alpha)) - \varphi(S_{min}) + \varphi(Iso(\alpha))}{2}}.
\]


\subsubsection{Tools for dealing with products of shapes}
\label{sec:product_rules}
As mentioned earlier, our analysis involves large powers the matrix $\Delta$. In the following, we will derive a graph matrix representation for $\Delta$. Unfortunately, explicitly writing down such a representation for $\Delta^k$ for arbitrary $k \in \N$ is complicated. To overcome this issue, we now introduce some definitions and technical results that allow us to express in a systematic way the graph matrix representation of a product of matrices in terms of the representations of the individual matrices.
\begin{definition}[Multiplication rule]
\label{defn:mult-rule}
Given shapes $\alpha$ and $\beta$ such that $V_{\alpha}$ and $U_{\beta}$ match (i.e. $V_{\alpha}$ and $U_{\beta}$ have the same number \aw{and order? or do circles always come first in the order?} of circle and square vertices), the product $M_{\alpha}M_{\beta}$ is a linear combination of graph matrices $M_\gamma$ of shapes $\gamma$ of the following form:
\begin{enumerate}
    \item Glue $\alpha$ and $\beta$ together by setting $V_{\alpha} = U_{\beta}$; these vertices now become middle vertices of $\gamma$. We take the $U_{\alpha}$ to be the left side of $\gamma$ and we take $V_{\beta}$ to be the right side of $\gamma$.
    \item The possible realizations of $\gamma$ are obtained considering all possible identification patterns of how the vertices in $V(\beta) \setminus U_{\beta}$ may intersect with the vertices in $V(\alpha) \setminus V_{\alpha}$ subject to the following two constraints:
    \begin{enumerate}
        \item Circle vertices can only be identified with other circle vertices and square vertices can only be identified with other square vertices.
        \item The vertices in $V(\alpha) \setminus V_{\alpha}$ must remain distinct as well as the vertices in $V(\beta) \setminus U_{\beta}$. In other words, each vertex can only be identified with one other vertex (which must be in the other shape).
    \end{enumerate}
    
    \item If there are multi-edges in $\gamma$ (i.e. two or more labeled edges with the same endpoints), convert them to a linear combination of labeled edges, as described below. We then re-express $M_\gamma$ as a linear combination of graph matrices, each of which corresponds to a graph obtained by picking one of the aforementioned labeled edges.
    
    The rule for converting multi-edges to a linear combination of labeled edges is as follows. If we have two parallel edges with labels $i$ and $j$ then we can replace these edges with a sum over $k \in \mathbb{N} \cup \{0\}$ of $c_{ijk}$ times an edge with label $k$ where $\{c_{ijk}: i,j,k \in \mathbb{N} \cup \{0\}\}$ are the coefficients such that 
    \[
    h_i(x)h_j(x) = \sum_{k = 0}^{\infty}{c_{ijk}h_k(x)}.
    \]
    A key property of the coefficients $c_{ijk}$ is that $c_{ijk} = 0$ unless $i + j + k$ is even. In other words, for each term we obtain, the parity of $k$ is the same as the parity of $i + j$.
\end{enumerate}
\end{definition}
\begin{lemma}\label{lem:multiplyHermitebyx}
For all $j \in \mathbb{N}$,
\[
h_1(x)h_j(x) = xh_{j}(x) = \sqrt{j+1}h_{j+1}(x) + \sqrt{j}h_{j-1}(x)
\]
where we are using the normalized Hermite polynomials.
\end{lemma}
\begin{proof}
Since the normalized Hermite polynomials $\{h_j: j \in \mathbb{N} \cup \{0\}\}$ are orthonormal with respect to the inner product 
\[
\langle{h_i,h_j}\rangle = E_{x \sim N(0,1)}[h_i(x)h_j(x)]
\]
we have that 
\[
xh_j(x) = \sum_{k = 0}^{\infty}{E_{y \sim N(0,1)}[yh_j(y)h_k(y)]h_k(x)}
\]
We now make the following observations:
\begin{enumerate}
    \item If $k < j-1$ then $E_{y \sim N(0,1)}[yh_j(y)h_k(y)] = 0$ because $yh_k(y)$ is a degree $k+1$ polynomial and $h_j(y)$ is orthogonal to all polynomials of degree less than $j$.
    \item If $k > j+1$ then $E_{y \sim N(0,1)}[yh_j(y)h_k(y)] = 0$ because $yh_j(y)$ is a degree $j+1$ polynomial and $h_k(y)$ is orthogonal to all polynomials of degree less than $k$.
    \item If $k = j$ then 
    $E_{y \sim N(0,1)}[yh_j(y)h_k(y)] = 0$ because $yh_j(y)h_k(y)$ is an odd polynomial.
    \item If $k = j-1$ then the leading term of $yh_k(y) = \frac{x^j}{\sqrt{(j-1)!}}$ so we can write $yh_k(y) = \sqrt{j}h_j(y) + p$ where $p$ has degree at most $j-1$. This implies that 
    $E_{y \sim N(0,1)}[yh_j(y)h_k(y)] = E_{y \sim N(0,1)}[\sqrt{j}(h_j(y))^2] = \sqrt{j}$
    \item If $k = j+1$ then the leading term of $yh_j(y) = \frac{x^k}{\sqrt{j!}}$ so we can write $yh_j(y) = \sqrt{j+1}h_{k}(y) + p$ where $p$ has degree at most $k-1$. This implies that 
    $E_{y \sim N(0,1)}[yh_j(y)h_k(y)] = E_{y \sim N(0,1)}[\sqrt{j+1}(h_{k}(y))^2] = \sqrt{j+1}$
\end{enumerate}
\end{proof}
\begin{corollary}
For all $j \in \mathbb{N}$,
\[
{x^2}h_{j}(x) = \sqrt{(j+1)(j+2)}h_{j+2}(x) + (2j+1)h_{j}(x) + \sqrt{j(j-1)}h_{j-2}(x)
\]
\end{corollary}
\begin{proof}
By Lemma \ref{lem:multiplyHermitebyx},
\begin{align*}
{x^2}h_{j}(x) &= x\sqrt{j+1}h_{j+1}(x) + x\sqrt{j}h_{j-1}(x) \\
&=\sqrt{j+1}(\sqrt{j+2}h_{j+2}(x) + \sqrt{j+1}h_{j}(x)) + \sqrt{j}(\sqrt{j}h_{j}(x) + \sqrt{j-1}h_{j-2}(x)) \\
&= \sqrt{(j+1)(j+2)}h_{j+2}(x) + (2j+1)h_{j}(x) + \sqrt{j(j-1)}h_{j-2}(x)
\end{align*}
\end{proof}
\begin{corollary}
For all $j \in \mathbb{N}$,
\[
h_2(x)h_{j}(x) = \frac{x^2 - 1}{\sqrt{2}}h_j(x) =  \sqrt{\frac{(j+1)(j+2)}{2}}h_{j+2}(x) + \sqrt{2}{j}h_{j}(x) + \sqrt{\frac{j(j-1)}{2}}h_{j-2}(x)
\]
\end{corollary}




\subsection{Some graph matrix representations}
\label{sec:shapes}
In this section, we derive the graph matrix representations of various matrices that arise in our analysis. For the purposes of computing ${\calA}{\calA}^{*}$, we can view $\calA$ as an $n \times d^2$ matrix $A$ with rows indexed by a single index in $[n]$ and columns indexed by an ordered pair of indices in $[d]$. With this view, we can decompose $A$ as $A = M_{\alpha_{A1}} + M_{\alpha_{A2}}$ and $A^{*} = M_{\alpha_{A1}}^T + M_{\alpha_{A2}}^T$ for the following shapes $\alpha_{A1}$ and $\alpha_{A2}$ (note that $\alpha_{A2}$ is improper). Here by improper, we mean that the shape contains a multi-edge. For every shape $\alpha$ considered below, its vertices are given by $U_\alpha \cup V_\alpha \cup W_\alpha$ (here we abuse notation and let $U_\alpha$ denote the union of all vertices in the tuple it contains, same for $V_\alpha$).




\begin{enumerate}
    \item $U_{\alpha_{A1}} = (u)$ where $u$ is a circle vertex, $V_{\alpha_{A1}} = (v_1,v_2)$ where $v_1,v_2$ are square vertices, $W_{\alpha_{A1}} = \{\}$ and $E(\alpha_{A1}) = \{\{u,v_1\}, \{u,v_2\}\}$.
    \item $U_{\alpha_{A2}} = (u)$ where $u$ is a circle vertex, $V_{\alpha_{A2}} = (v,v)$ where $v$ is a square vertex, $W_{\alpha_{A2}} = \{\}$ and $E(\alpha_{A2}) = \{\{u,v\}, \{u,v\}\}$.
\end{enumerate}

Insert picture here.

Multiplying $A$ and $A^{*}$, we have the following decomposition for ${\calA}{\calA}^{*} = {A}A^{*}$.
\[
{\calA}{\calA}^{*} = M_{\alpha_1} + M_{\alpha_2} + M_{\alpha_3} + M_{\alpha_4}
\]
where $\alpha_1$, $\alpha_2$, $\alpha_3$, and $\alpha_4$ are the following shapes (note that $\alpha_2$, $\alpha_3$, and $\alpha_4$ are improper):

\pax{The notation `$w$' was way overloaded, so I changed the name of an interior vertex in a shape to be called `$x$' instead. For consistency I also changed $w_1, w_2$ to $x_1, x_2$.}

\begin{enumerate}
    \item $U_{\alpha_{1}} = (u)$ and  $V_{\alpha_{1}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{1}} = \{x_1,x_2\}$ where $x_1,x_2$ are square vertices, and $E(\alpha_{1}) = \{\{u,x_1\}, \{u,x_2\}, \{x_1,v\},\{x_2,v\}\}$.
    \item $U_{\alpha_{2}} = (u)$ and  $V_{\alpha_{2}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{2}} = \{x\}$ where $x$ is a square vertex, and $E(\alpha_{2}) = \{\{u,x\}, \{u,x\}, \{x,v\},\{x,v\}\}$.
    \item $U_{\alpha_{3}} = V_{\alpha_{3}} = (u)$ where $u$ is a circle vertex, $W_{\alpha_{3}} = \{x_1,x_2\}$ where $x_1,x_2$ are square vertices, and $E(\alpha_{3}) = \{\{u,x_1\}, \{u,x_1\}, \{u,x_2\}, \{u,x_2\}\}$.
    \item $U_{\alpha_{4}} = V_{\alpha_{4}} = (u)$ where $u$ is a circle vertex, $W_{\alpha_{4}} = \{x\}$ where $x$ is a square vertex, and $E(\alpha_{4}) = \{\{u,x\}, \{u,x\}, \{u,x\},\{u,x\}\}$.
\end{enumerate}
Insert picture here

To shift from improper shapes (i.e. ones with multi-edges) to proper shapes (i.e. ones without multi-edges), we make the following observations and invoke the rule described in Definition~\ref{defn:mult-rule}. For $x \in \R$, we have
\begin{enumerate}
    \item $x^2 = (x^2 - 1) + 1 = \sqrt{2}h_2(x) + 1$
    \item $x^4 = (x^4 - 6x^2 + 3) + 6(x^2 - 1) + 3 = \sqrt{24}h_4(x) + 6\sqrt{2}h_2(x) + 3$
\end{enumerate}
We now have that 
\begin{align*}
{\calA}{\calA}^{*} &= M_{\alpha_1} + 2M_{\alpha_{2a}} + \sqrt{2}M_{\alpha_{2b}} + \sqrt{2}M_{\alpha_{2c}} + dM_{\alpha_{2d}} + 2M_{\alpha_{3a}} + 2\sqrt{2}(d-1)M_{\alpha_{3b}} + (d^2 - d)M_{\alpha_{3c}} \\
&+ \sqrt{24}M_{\alpha_{4}} + 6\sqrt{2}M_{\alpha_{3b}} + 3dM_{\alpha_{3c}}   
\end{align*}
where $\alpha_1$, $\alpha_{2a}$, $\alpha_{2b}$, $\alpha_{2c}$, $\alpha_{2d}$, $\alpha_{3a}$, $\alpha_{3b}$, $\alpha_{3c}$, and $\alpha_{4}$ are the following proper shapes (note that the definition of $\alpha_4$ changes from above):
\begin{enumerate}
    \item $\alpha_1$ is the same as above.
    \item $U_{\alpha_{2a}} = (u)$ and  $V_{\alpha_{2a}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{2a}} = \{x\}$ where $x$ is a square vertex, and $E(\alpha_{2a}) = \{\{u,x\}_2, \{x,v\}_2\}$.
    \item $U_{\alpha_{2b}} = (u)$ and  $V_{\alpha_{2b}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{2b}} = \{x\}$ where $x$ is a square vertex, and $E(\alpha_{2b}) = \{\{u,x\}_2\}$.
    \item $U_{\alpha_{2c}} = (u)$ and  $V_{\alpha_{2c}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{2c}} = \{x\}$ where $x$ is a square vertex, and $E(\alpha_{2c}) = \{\{x,v\}_2\}$.
    \item $U_{\alpha_{2d}} = (u)$ and  $V_{\alpha_{2d}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{2d}} = \{\}$, and $E(\alpha_{2d}) = \{\}$.
    \item $U_{\alpha_{3a}} = V_{\alpha_{3a}} = (u)$ where $u$ is a circle vertex, $W_{\alpha_{3a}} = \{x_1,x_2\}$ where $x_1,x_2$ are square vertices, and $E(\alpha_{3a}) = \{\{u,x_1\}_2, \{u,x_2\}_2\}$.
    \item $U_{\alpha_{3b}} = V_{\alpha_{3a}} = (u)$ where $u$ is a circle vertex, $W_{\alpha_{3b}} = \{x\}$ where $x$ is a square vertex, and $E(\alpha_{3b}) = \{\{u,x\}_2\}$.
    \item $U_{\alpha_{3c}} = V_{\alpha_{3c}} = (u)$ where $u$ is a circle vertex, $W_{\alpha_{3c}} = \{\}$, and $E(\alpha_{3c}) = \{\}$.
    \item $U_{\alpha_{4}} = V_{\alpha_{4}} = (u)$ where $u$ is a circle vertex, $W_{\alpha_{4}} = \{x\}$ where $x$ is a square vertex, and $E(\alpha_{4}) = \{\{u,x\}_4\}$.
\end{enumerate}

\TODO{Insert picture here.}

Since $M_{\alpha_{2d}} = 1_{n}1_{n}^T - I_n$ and $M_{\alpha_{3c}} = I_n$, we have that
\[
{\calA}{\calA}^{*} = (d^2 + d)I_{n} + d{1_n}{1_n^T} + M_{\alpha_1} + 2M_{\alpha_{2a}} + \sqrt{2}M_{\alpha_{2b}} + \sqrt{2}M_{\alpha_{2c}} + 2M_{\alpha_{3a}} + (2\sqrt{2}d + 4\sqrt{2})M_{\alpha_{3b}} + \sqrt{24}M_{\alpha_{4}}.
\]
In order to decompose $B = {\calA}{\calA}^{*} - W$ in terms of graph matrices, we also need to decompose $W$ in terms of graph matrices. This decomposition is as follows:
\[
W = w{1_n}^T + 1_{n}w^T + d{1_n}{1_n}^T = \sqrt{2}M_{\alpha_{2b}} + \sqrt{2}M_{\alpha_{2c}} + 2\sqrt{2}M_{\alpha_{3b}} + d{1_n}{1_n}^T.
\]
Combining these decompositions, we have that:
\begin{align}
    \label{eqn:Bdef}
    B &= \calA \calA^* - W = (d^2 + d)I_{n} + M_{\alpha_1} + 2M_{\alpha_{2a}} +  2M_{\alpha_{3a}} + (2\sqrt{2}d + 2\sqrt{2})M_{\alpha_{3b}} + \sqrt{24}M_{\alpha_{4}}, \text{ and } \\
    \Delta &= -M_{\alpha_1} -2M_{\alpha_{2a}} - 2M_{\alpha_{3a}} - (2\sqrt{2}d + 2\sqrt{2})M_{\alpha_{3b}} - \sqrt{24}M_{\alpha_{4}}
    \label{eqn:Delta_def} 
\end{align}


Define the index set $\calI = \{1,2a,3a,3b,4\}$, which collects the indices of non-identity shapes appearing in $B$. For a given index $i \in \calI$, we define $\lambda_i$ to be the scalar coefficient appearing in front of $M_{\alpha_i}$ in the expression for $B$ above. 

We also express the each vector $w, 1_n \in \R^n$ (recall $w_i = \| v_i \|_2^2 - d$) as an $n \times 1$ graph matrix. We have that $w$ is represented by the shape $\alpha_w$ defined as follows, which has leading coefficient $\sqrt{2}$, and $1_n$ is represented by the shape $\alpha_{1_n}$ with leading coefficient $1$.

\begin{enumerate}
    \item $U_{\alpha_w} = (u)$ where $u$ is a circle vertex, $V_{\alpha_w} = \emptyset$, $W_{\alpha_w} = \{x_1\}$ where $x_1$ is a square vertex, and $E(\alpha_w) = \{ \{u, x_1\}_2 \}$.
    \item $U_{\alpha_{1_n}} = (u)$ where $u$ is a circle vertex, $V_{\alpha_{1_n}} = \emptyset$, and $E(\alpha_{1_n}) = \emptyset$. 
\end{enumerate}

\pax{To do: insert pictures}

We also define $\alpha_{A^{*},1}$, $\alpha_{A^{*},2}$, and $\alpha_{A^{*},3}$ to be the shapes such that
\begin{enumerate}
    \item $U_{\alpha_{A^{*},1}} = (u)$ and  $V_{\alpha_{A^{*},1}} = (v)$ where $u, v$ are square vertices, $W_{\alpha_{A^{*},1}} = \{x\}$ where $x$ is a circle vertex, and $E(\alpha_{A^{*},1}) = \{\{u,x\}, \{x,v\}\}$.
    \item $U_{\alpha_{A^{*},2}} = V_{\alpha_{A^{*},2}} = (u)$ where $u$ is a square vertex, $W_{\alpha_{A^{*},2}} = \{x\}$ where $x$ is a circle vertex, and $E(\alpha_{A^{*},2}) = \emptyset$.
    \item $U_{\alpha_{A^{*},3}} = V_{\alpha_{A^{*},3}} = (u)$ where $u$ is a square vertex, $W_{\alpha_{A^{*},3}} = \{x\}$ where $x$ is a circle vertex, and $E(\alpha_{A^{*},3}) = \{\{u,x\}_2\}$.
\end{enumerate}
% Recall that $\alpha_{w}$ is the shape such that 
% $U_{\alpha_{w}} = (u)$ and $V_{\alpha_{w}} = \emptyset$ where $u$ is a circle vertex, $W_{\alpha_{w}} = \{x\}$ where $x$ is a square vertex, and $E(\alpha_{w}) = \{\{u,x\}_2\}$.
% \end{definition}
The previous shapes are useful in that they represent the action of $\calA^*$ on a given vector: the terms arising in $\calA^* x$ for $x \in \R^n$ are obtained by appending (according to rules explained in Section \ref{sec:product_rules}) the graph matrix representation of $x$ to one of $\alpha_{A^*,j}$ for $j \in \{1,2,3\}$
%\aw{with some coefficients?}. 
See Section \ref{sec:normbound_strat} for details. 
% These shapes arise on the left of $\calA^* \Delta^k 1_n$, $\calA^* \Delta^k w$, and $1^T \Delta^k w$. See Section {sec:normbound_strat}.

\TODO{Insert pictures here.}

Given these graph matrix representations, we can immediately prove Lemma~\ref{lemma:B-concentrates}.


\begin{proof}[Proof of Lemma~\ref{lemma:B-concentrates}]
	
	
	
Recall that for $a \in \alpha$, we have $\varphi(a) = \log_n(n)=1$ if $a$ is a circle and $\varphi(a) = \log_n(d) \approx 1/2$ if $a$ is a square (since we consider the regime $n  d^2/\polylog(d)$). Recall that $Iso(\alpha)$ is the set of isolated vertices that do not lie in $U_\alpha$ or $V_\alpha$.

\aw{recall eq number with $B$'s expansion in terms of shapes?} \pax{Done, thanks}
\aw{I meant that here we should give some overview of what we're doing before diving into case-work}

    
 
For $\alpha_1$, consider the following vertex separators: $\{ u\}, \{ v \}, \{ x_1, x_2 \}$. By inspection, any other vertex separator contains one of these three. The weights of $\{ u\}$  and $\{ v \}$ are both $1$. The weight of $\{ x_1, x_2\}$ is $2\log_n(d) > 1$. Thus we may choose $u$ as a min-vertex separator without loss of generality. Thus for $\alpha = \alpha_1$, we have
	\[
	\frac{\varphi(V(\alpha)) - \varphi(S_{min}) + \varphi(Iso(\alpha))}{2}
	= \frac{ (2 \log_n(d) + 2) - 1 + 0 }{2} 
	= \frac{2 \log_n(d) + 1}{2},
	\]
	leading to a norm bound $\|M_{\alpha_1}\|_{op} = \tilde O( d\sqrt{n})$ with high probability by Theorem \ref{thm:graph-matrix-norm-bound}. 
	
	% On removing $u$, the vertices $v, x_1, x_2$ are nonisolated, leading to a norm bound of $\tilde O(d \sqrt{n}$, with high probability by Theorem \ref{thm:graph-matrix-norm-bound}.
	
	Next consider $\alpha_2$. Every vertex is a separator of $U_{\alpha_2}$ and $V_{\alpha_2}$. Since $x$ has weight $\log_n(d)<1$ and $u, v$ have weight $1$ in $\alpha_2$, the minimum weight vertex separator is $x$. Thus for $\alpha = \alpha_2$, we have
	\[
	\frac{\varphi(V(\alpha)) - \varphi(S_{min}) + \varphi(Iso(\alpha))}{2}
	= \frac{  ( 2 + \log_n(d)  ) - \log_n(d) + 0}{2}
	= 1,
	\] 
	leading to a high probability norm bound $\|M_{\alpha_2}\|_{op} = \tilde O(n)$ by Theorem \ref{thm:graph-matrix-norm-bound}.
	
	% On removing $x$, the remaining circle vertices are isolated, which leads to a norm bound of $\tilde O(n)$ with high probability by Theorem \ref{thm:graph-matrix-norm-bound}.
	
	The remaining shapes represent matrices that are diagonal; thus $u$ is the min-vertex separator. For $\alpha_{3a}$, 
	% $u$ must be removed to separate $U_{\alpha_{3a}}$ and $V_{\alpha_{3a}}$. 
	by similar arguments to the above,  Theorem \ref{thm:graph-matrix-norm-bound} yields $\| M_{\alpha_{3a}} \| =  \tilde O( d ) $. For $\alpha_{3b}$, we obtain a norm bound $\tilde O( n^{(1+ \log_n d - 1 + 0)/2} = \tilde O( d^{1/2} )$, so its contribution to $\Delta$ has operator norm at most $\tilde O(d^{3/2})$ (see \eqref{eqn:Delta_def}). Similarly, we obtain the norm bound $\tilde O( d^{1/2})$ for $\alpha_4$, completing the proof.
\end{proof}




\subsection{Norm Bound Strategy Using Graph Matrices}
\label{sec:normbound_strat}
We need to bound norms of matrices of the following forms: \aw{in the lemmas stated earlier we removed the scalar factors $\alpha$, so we can do away with those throughout this section? this would help alleviate the double meaning of $\alpha$ too...}
\begin{enumerate}
    \item $\{\mathcal{A}^{*}{({\alpha}^{-1}\Delta)^k}w:  k \in \mathbb{N}\}$ 
    \item $\{\mathcal{A}^{*}{({\alpha}^{-1}\Delta)^k}{1_n}: k \in \mathbb{N}\}$
    \item $\{{1_n}^T{({\alpha}^{-1}\Delta)^k}w: k \in \mathbb{N}\}$. (Here, we regard the scalars as $1 \times 1$ matrices.)
\end{enumerate}

For a fixed $k$, consider one of the matrices in 1--3. In Section \ref{sec:shapes}, we express $\calA^*$ and $\Delta$ as a linear combination of shapes. Thus, for fixed $k$, any matrix in 1--3 above can be written as linear combination of terms, where each term is a product of shapes, say 
\begin{align}
\label{eqn:general_product}
    M_{\beta_{start}} \cdot M_{ \beta_1} \cdots M_{\beta_k} \cdot M_{\beta_{end}},
\end{align} where each $\beta_i$ is a (proper) shape from Section \ref{sec:shapes}. For each term as in \eqref{eqn:general_product}, we further decompose it into a linear combination of several sub-terms represented by new (proper) shapes. Let $\alpha_{P}$ denote a shape that arises as a subterm. Then the shape $\alpha_{P}$ can be constructed by the following procedure: 

% For any fixed $k$, when we expand out these expressions, we obtain a various terms that are products of shapes coming from $\calA^*, \Delta, 1_n$ and $w$, each of which is obtained through the following procedure.  

\begin{enumerate}
    % \item Each term as in \eqref{eqn:general_product} arises from the product of $k+2$ shapes $\beta_{start}, \beta_1, \ldots, \beta_{k}, \beta_{end}$, where
    % $\beta_{start}$ is one of $\alpha_{A^{*},1}$, $\alpha_{A^{*},2}$,  $\alpha_{A^{*},3}$, or $I_n$, $\beta_1,\ldots,\beta_{k}$ are shapes in $\{\alpha_i: i \in \calI\}$ (coming from $\Delta$), and $\beta_{end}$ is one of $\alpha_{1_n}$ or $\alpha_{w}$. 

    \item We start with $\beta_{start}$. If $\beta_{start}$ is $\alpha_{A^{*},1}$, $\alpha_{A^{*},2}$, or $\alpha_{A^{*},3}$, we call the circle vertex $x$ to be the (initial) \textit{loose end}. If $\beta_{start} = \alpha_{1_n^T}$, we call the single  vertex in this shape, which is a circle, the (initial) \textit{loose end}. In all cases, we set $U_{\alpha_P} = U_{\beta_{start}}$ and $V_{\alpha_P} = V_{\beta_{start}} $. (Note the $U_{\alpha_{P}} = V_{\alpha_{P}} = \emptyset$ if $\beta_{start} = \alpha_{1_n^T}$.
    
    % If $\beta_{start} = \alpha_{1_n^T}$, instead of having the circle vertex be in $V$, we make $U$ and $V$ empty and call the circle vertex to be the (initial) \textit{loose end}.

    \item We now do the following for each $j \in [k]$  
    \begin{enumerate}
        \item[(a)] Append the shape $\beta_{j}$ by identifying $U_{\beta_j} = (u)$ with the current loose end and making $V_{\beta_j} = (v)$ the new loose end.
        \item[(b)] For each vertex in $V(\beta_j) \setminus U_{\beta_j}$, either leave it alone or identify it with an existing vertex of the same type (circle or square) which is not $u$ and has not yet been identified with a vertex in $V(\beta_j) \setminus U_{\beta_j}$.
        \item[(c)] If this creates two parallel edges with integer labels $N$ and $M$, we either (i) remove these parallel edges if $N+M$ is even or (ii) replace those parallel edges with a single labeled edge that has the same parity as $N+M$ and lies in $[N+ M]$. 

        In either case (i) or (ii), assign the edge (or empty edge) a coefficient according to the rule in Definition~\ref{defn:mult-rule}. \pax{This part is a bit awkward to state for nonedges}
        
        % In and that is assigned a \textit{coefficient} according to the 
                
        % Whenever we have two parallel labeled edges, replace them with a single labeled edge (which could have label $0$, in which case the edge vanishes) as in the rule described in Definition~\ref{defn:mult-rule}. The parity of the resulting label will be the same as the parity of the sum of the original labels.
    \end{enumerate}

    \item Finally, apply the same procedure as described in 2(a--c) to $\beta_{end}$.

    Concretely, if the last term in the product is $1_n$ (so $\beta_{end} = \alpha_{1_n}$), we stop here. If the last term in the product is $w$ (so $\beta_{end} = \alpha_{w}$), we append $\alpha_w$ to the existing shape by identifying the current loose end with $U_{\alpha_w} = (u)$. Then, for each set of resulting parallel edges, we remove or replace them as described in 2(c) and assign them coefficients.
    
    % Recalling $W_{\alpha_w} = \{x\}$, we then either leave $x$ alone or identify it with an existing vertex which is not $u$. If this creates two parallel edges with integer labels $N$ and $M$, we replace them with a single labeled edge that has the same parity as $N+M$, that lies in $[N+ M]$, and that is assigned a coefficient according to the rule in Definition~\ref{defn:mult-rule}. 
    
    % \item We apply this same procedure for $\beta_{end}$ as in 2. except that since $V_{\beta_{end}} = \emptyset$, we tie up the loose end instead of creating a new loose end. 
    
    % In other words, if the last term in the product is $1_n$ (so $\beta_{end} = \alpha_{1_n}$), we stop here (tying up the loose end). If 

    % \item Define 
 
\end{enumerate}

As we described, the matrices $\calA^*(\alpha^{-1} \Delta)^k w, \calA^*(\alpha^{-1} \Delta)^k 1_n$ and $1_n^T (\alpha^{-1} \Delta^k) w$ are linear combinations of terms of the form $\alpha_{P}$. We now describe the coefficients associated to a particular term $\alpha_P$ in this linear combination. To do so we introduce two definitions.
% regarding these product terms. 
\begin{definition}
For each shape $\beta_j$ for $j \in [k]$, we define its \textbf{coefficient} $c(\beta_j)$ to be its coefficient in the graph matrix decomposition of  $\alpha^{-1} \Delta$.
\end{definition}

\begin{definition}
Given shapes $\beta_{start}, \beta_1, \ldots, \beta_{k}, \beta_{end}$ as described above, an \textbf{identification pattern} $P$ on $\beta_{start}, \beta_1, \ldots, \beta_{k}, \beta_{end}$ specifies which vertices are identified with each other (beyond the automatic identifications, such as identifying $V_{\beta_t}$ with $U_{\beta{t+1}}$) and which labelled edge is chosen when we convert parallel labeled edges into a single labeled edge according to the rule in Definition~\ref{defn:mult-rule} as in step 2(c) above. We define $\mathcal{P}_{\beta_{start}, \beta_1, \ldots, \beta_{k}, \beta_{end}}$ to be the set of all identification patterns on the shapes $\beta_{start}, \beta_1, \ldots, \beta_{k}, \beta_{end}$.

Given an identification pattern $P$, we define $\alpha_{P}$ to be the shape resulting from $P$ and we define $c_{P}$ to be the coefficient, so that the resulting  term is ${c_P}\cdot \prod_{j=1}^{k}{c(\beta_j)} \cdot M_{\alpha_P}$.

In other words, $c_P$ captures the part of the coefficient of $M_{\alpha_P}$ which comes from converting parallel labeled edges into a single labeled edge (or non-edge). \aw{I guess the coefficients coming from $\beta_{start}$ and $\beta_{end}$ are also absorbed into $c_P$? e.g., there's a factor of $\sqrt{2}$ associated with $w$; but these are all constants (not depending on $n,d$) so they don't really matter}
\end{definition}
With these definitions and for a fixed 
% $\beta_{start}$, $\beta_{end}$, and 
$k$, each of $\calA^*(\alpha^{-1} \Delta^k 1_n), \calA^*(\alpha^{-1} \Delta^k w)$ and $1_n^T(\alpha^{-1} \Delta^k) w$ can each be expressed as a summation of the following form:
\begin{align} 
\label{eqn:pattern_decomposition} 
\sum_{\beta_1,\ldots,\beta_k \in \{\alpha_i: i \in \calI\}} \, \, {\sum_{P \in \mathcal{P}_{\beta_{start},\beta_1,\ldots,\beta_k,\beta_{end}}}{\bigg( {c_P}\cdot \prod_{j=1}^{k}{c(\beta_j)} \bigg) M_{\alpha_P}}}
\end{align} 
To bound the norm of this expression, we apply the triangle inequality and bound separately $\norm{M_{\alpha_P}}_{op}$ for each identification pattern $P$.
\subsubsection{Upper bounding $\norm{M_{\alpha_P}}_{op}$ via weights}
\label{sec:norm-bounds-via-weights}
In order to upper bound $\norm{M_{\alpha_P}}_{op}$, we will try and consider the contribution to $\norm{M_{\alpha_P}}_{op}$ from each of the shapes $\beta_{start},\beta_1,\ldots,\beta_k,\beta_{end}$. In order to invoke the bound in Theorem~\ref{thm:graph-matrix-norm-bound}, we must be able to calculate the min-vertex separator of $\alpha_P$ and status (i.e. square vs. circle and isolated vs. non-isolated) of each of the vertices of $\alpha_P$. Specifically, define the following short-hand notation for the dominant term in the norm bound of Theorem~\ref{thm:graph-matrix-norm-bound}:
\[
N_\approx(\alpha_P) = n^{\frac{\varphi(V(\alpha_P)) - \varphi(S_{min}) + \varphi(Iso(\alpha_P))}{2}}
\]
where $S_{min}$ is a min-vertex separator of $\alpha_P$.

To compute the combinatorial quantities that define $N_{\approx}(P)$, we will design an ideal weight function $w_{ideal,P}$ and an actual weight function $w_{actual,P}$, each of which assigns a \textit{weight} to each of the shapes 
$\beta_{start},\beta_1,\ldots,\beta_k,\beta_{end}$. Intuitively, the ideal weight function allows us to accurately estimate the right-hand side of the norm bound in Theorem~\ref{thm:graph-matrix-norm-bound}. However, as we explain later, determining this ideal weight function exactly is intractable. Instead, we show that the actual weight function is a faithful ``relaxation'' of the ideal weight function, tractable to calculate and still leads to sufficiently good norm bounds. 

More precisely, the following properties must be satisfied: 
\begin{enumerate}
    \item  $N_{\approx}(\alpha_P) = \prod_{j=0}^{k+1}{w_{ideal,P}(\beta_{j})}$ where $\beta_{0} = \beta_{start}$ and $\beta_{k+1} = \beta_{end}$. This ensures that the product of the ideal weights over the shapes $\beta_j$ faithfully estimates the dominant term of the norm bound in Theorem~\ref{thm:graph-matrix-norm-bound}.
    \item $\prod_{j=0}^{k+1}{w_{actual,P}(\beta_{j})} \geq \prod_{j=0}^{k+1}{w_{ideal,P}(\beta_{j})}$. In fact, for almost all shapes $\beta_j$ we will have that \\ $w_{actual,P}(\beta_{j}) \geq w_{ideal,P}(\beta_{j})$. This ensures that the actual weight function gives a norm bound that is valid (i.e. no smaller than the ``true'' norm bound given by the ideal weight function).
    \item For all $j \in [k]$, $|w_{actual,P}(\beta_j)c(\beta_j)| \leq \frac{\sqrt[4]{n}}{\sqrt{d}}$. This ensures that the norm bound given by the actual weight function is sufficiently small to complete the proofs of our technical lemmas.
\end{enumerate}
We note that the number of possibilities for $\beta_1,\ldots,\beta_k$, the number of possible identification patterns on $\beta_{start},\beta_1,\ldots,\beta_k,\beta_{end}$, the maximum coefficient $c_P$ for any identification pattern $P$, and the ratio $\frac{\norm{M_{\alpha_P}}_{op}}{N_{\approx}(\alpha_P)}$ (assuming probabilistic norm bound in Theorem~\ref{thm:graph-matrix-norm-bound} holds) are all at most $\polylog(n)^{O(k)}$. This follows from the observation that we have $k+2$ shapes $\beta_{start},\beta_1,\ldots,\beta_k,\beta_{end}$, each consisting of $O(1)$ vertices and edges, and a simple combinatorial fact which we defer to the appendix (Proposition~\ref{prop:number-of-shapes-bound}).

Thus, if we can specify weight functions satisfying the above properies, then:
\begin{align*}
    &\sum_{\beta_1,\ldots,\beta_k \in \{\alpha_i : i \in \calI\}}{\sum_{P \in \mathcal{P}_{\beta_{start},\beta_1,\ldots,\beta_k,\beta_{end}}}{{|c_P|}\left(\prod_{j=1}^{k}{|c(\beta_j)|}\right)\norm{M_{\alpha_P}}_{op}}} \\
    &=\sum_{\beta_1,\ldots,\beta_k}{\sum_{P \in \mathcal{P}_{\beta_{start},\beta_1,\ldots,\beta_k,\beta_{end}}}{{|c_P|}\left(\prod_{j=1}^{k}{|c(\beta_j)|}\right)\left(\prod_{j=0}^{k+1}{w_{ideal,P}(\beta_j)}\right)\frac{\norm{M_{\alpha_P}}_{op}}{N_{\approx}(\alpha_P)}}} \\
    &\leq \left(\frac{\sqrt[4]{n}\, \polylog(n)}{\sqrt{d}}\right)^{k}\max_P{\{w_{actual,P}(\beta_{start})w_{actual,P}(\beta_{end})\}}.
\end{align*}
\subsubsection{Minimum weight vertex separator of $\alpha_P$}
Before specifying the weight functions, we recall that:
\begin{align*}
N_{\approx}(\alpha_P) = &d^{\frac{|V_{\Box}(\alpha_P)| + (\# \text{ of isolated vertices in } V_{\Box}(\alpha_P)) - (\# \text{ of square vertices in } S) }{2}} \\
&n^{\frac{|V_{\circ}(\alpha_P)| + (\# \text{ of isolated vertices in } V_{\circ}(\alpha_P)) - (\# \text{ of circle vertices in } S) }{2}}
\end{align*}
where $S$ is a minimum weight vertex separator of $\alpha_P$. We now determine the minimum weight vertex separator for $\alpha_P$.

When $\beta_{start} = \alpha_{1_n^T}$, $U_{\alpha_P} = V_{\alpha_P} = \emptyset$ so $S = \emptyset$. As we now show, when $\beta_{start}$ is $\alpha_{A^{*},1}$, $\alpha_{A^{*},2}$, or $\alpha_{A^{*},3}$, the minimum weight vertex separator of $\alpha_P$ has a single square.
\begin{lemma}
\label{lem:min-vertex-sep}
If $\beta_{start}$ is $\alpha_{A^{*},1}$, $\alpha_{A^{*},2}$, or $\alpha_{A^{*},3}$ then the minimum weight vertex separator of $\alpha_P$ has a single square.
\end{lemma}
\begin{proof}
Since $U_{\alpha_P}$ consists of a single square and is a vertex separator, the minimum weight vertex separator is either a single square or no vertices at all. To show that the minimum weight vertex separator has at least one vertex, we prove that $U_{\alpha_P}$ must be connected to $V_{\alpha_P}$.

To prove this, it is sufficient to prove the following lemma. Here by `degree' of a vertex $a$ in a shape, we mean the sum of all edge labels of edges incident to $a$. 
\begin{lemma}\label{lem:connectivitylemma}
If $\beta_{start}$ is $\alpha_{A^{*},1}$, $\alpha_{A^{*},2}$, or $\alpha_{A^{*},3}$ then either $U_{\alpha_P} = V_{\alpha_P} = (u)$ where $u$ is a square vertex or $U_{\alpha_P} = (u)$, $V_{\alpha_P} = (v)$ where $u$ and $v$ are distinct square vertices and $u$ and $v$ are the only vertices with odd degree.
\end{lemma}
With this lemma, the result follows easily. If $U_{\alpha_P} = V_{\alpha_P} = (u)$ then the result is trivial. If $U_{\alpha_P} = (u)$ and $V_{\alpha_P} = (v)$ where $u$ and $v$ are distinct square vertices and are the only vertices with odd degree then $u$ and $v$ must be in the same connected component of $\alpha_P$ due to the following fact.
\begin{proposition}
\label{prop:handshake}
For any undirected graph $G$ with integer edge-labels, for any connected component $C$ of $G$, $\sum_{v \in C}{deg(v)}$ is even.
\end{proposition}
\begin{proof}
This is the handshaking lemma and can be proved by observing that $\sum_{v \in C}{deg(v)} = 2|E(C)|$ which is even.
\end{proof}

To be concrete, suppose that for the sake of contradiction $u$ and $v$ lie in distinct connected components $C_u$ and $C_v$ of $\alpha)_P$. Then the sum of degrees in $C_u$ is odd by Lemma \ref{lem:connectivitylemma}. But this contradicts Proposition \ref{prop:handshake}.

We proceed to prove Lemma \ref{lem:connectivitylemma}.
\begin{proof}[Proof of Lemma \ref{lem:connectivitylemma}]
Let $U_{\alpha_P} = (u)$ and $V_{\alpha_P} = (v)$. We make the following observations about the process for building the shape $\alpha_{P}$
\begin{enumerate}
    \item In $\beta_{start}$, either $u = v$ (in which case $u$ has even degree) or $u$ and $v$ are distinct square vertices which have odd degree. The circle vertex in $\beta_{start}$ always has even degree.
    
    \item For all of the shapes $\beta_1, \ldots, \beta_{k}, \beta_{k+1}$, all of the vertices have even degree.




    
    \item Whenever two vertices are identified, the parity of the degree of the resulting vertex is equal to the parity of the sum of the degrees of the original vertices.
    
    \item No other operation affects the parities of the degrees of the vertices.

\end{enumerate}
Together, these observations imply that either $u = v$ or $u$ and $v$ are the only vertices with odd degree. 
\end{proof} 
\end{proof}
\begin{corollary}\label{cor:alphaPapproximatenorm}
If $\beta_{start}$ is $\alpha_{A^{*},1}$, $\alpha_{A^{*},2}$, or $\alpha_{A^{*},3}$ then 
\[
N_{\approx}(\alpha_P) = d^{\frac{|V_{\Box}(\alpha_P)| + (\# \text{ of isolated vertices in } V_{\Box}(\alpha_P)) - 1}{2}} n^{\frac{|V_{\circ}(\alpha_P)| + (\# \text{ of isolated vertices in } V_{\circ}(\alpha_P))}{2}}
\]
If $\beta_{start}$ is $\alpha_{{1_n}^T}$ then 
\[
N_{\approx}(\alpha_P) = d^{\frac{|V_{\Box}(\alpha_P)| + (\# \text{ of isolated vertices in } V_{\Box}(\alpha_P))}{2}} n^{\frac{|V_{\circ}(\alpha_P)| + (\# \text{ of isolated vertices in } V_{\circ}(\alpha_P))}{2}}
\]
\end{corollary}
We remark that the factor of $\frac{1}{\sqrt{d}}$ appearing in the first expression turns out to be crucial to obtaining satisfactory norm bounds.

\subsubsection{The ideal weight function}
Given that we have identified the min-vertex separator of the shape $\alpha_P$, we now specify an ideal weight function $w_{ideal,P}$ such that $N_{\approx}(\alpha_P) = \prod_{j=0}^{k+1}{w_{ideal,P}(\beta_{j})}$. Each vertex $v$ in $V(\alpha_P)$, has an associated  value (i.e. $\sqrt{n}$ and $\sqrt{d}$ for non-isolated circles and squares, $n$ and $d$ for isolated circles and squares). We ``split'' this value among (at most) 2 shapes that contain $v$ by assigning the square root of the value of $v$ to $\beta_j$, where $j$ is the smallest index for which this vertex appears in $\beta_j$ and assigning the square root of the value of $v$ to $\beta_{j'}$ where $j'$ is the largest index for which this vertex appears in $\beta_{j'}$. If $v$ only appears once, then we assign the full value of $v$ to the shape in which it appears. Formally, we define this procedure in the following way. 
\begin{definition}
For each vertex $v \in V(\alpha_P)$, we define $w_{ideal,P}(v)$ so that 
\begin{enumerate}
    \item If $v$ is a square vertex which is not isolated then $w_{ideal,P}(v) = \sqrt{d}$.
    \item If $v$ is an isolated square vertex (note that vertices in $U_{\alpha_P} \cup V_{\alpha_P}$ do not count as isolated) then $w_{ideal,P}(v) = d$.
    \item If $v$ is a circle vertex which is not isolated then $w_{ideal,P}(v) = \sqrt{n}$
    \item If $v$ is an isolated circle vertex then $w_{ideal,P}(v) = n$ 
\end{enumerate}
\end{definition}
\begin{definition}
For $j \in [k+1]$, we define 
\[
w_{ideal,P}(\beta_j) = \prod_{v \in V(\beta_j)}{w_{ideal,P}(v)^{1 - \frac{1}{2} \I \{v \text{ appears in } \beta_{j'} \text{ for some } j' < j\} - \frac{1}{2} \I \{v \text{ appears in } \beta_{j'} \text{ for some } j' > j\}}}.
\]
For $\beta_0$, we adjust this to take the minimum weight vertex separator into account. In particular, if $\beta_0 = \alpha_{1_n^T}$ then 
\[
w_{ideal,P}(\beta_0) = \prod_{v \in V(\beta_0)}{w_{ideal,P}(v)^{1  - \frac{1}{2} \I \{v \text{ appears in } \beta_{j} \text{ for some } j > 0\}}}.
\]
while if $\beta_0$ is $\alpha_{A^{*},1}$, $\alpha_{A^{*},2}$, or $\alpha_{A^{*},3}$ then 
\[
w_{ideal,P}(\beta_0) = \frac{1}{\sqrt{d}}\prod_{v \in V(\beta_0)}{w_{ideal,P}(v)^{1  - \frac{1}{2}\I\{v \text{ appears in } \beta_{j} \text{ for some } j > 0\}}}.
\]
Note that for $j \geq 1$, vertices in $U_{\beta_j}$ automatically appear in $\beta_{j-1}$ and for $j < k+1$, vertices in $V_{\beta_j}$ automatically appear in $\beta_{j+1}$.
\end{definition}
\subsubsection{The local weight function and intuition for the actual weight function}
\label{sec:local_weights} 
Unfortunately, the ideal weight function cannot be computed separately for each shape $\beta_j$ because in order to determine if a vertex in $\beta_j$ is isolated or not, we need to consider the entire identification pattern $P$.

To handle this, we instead use a different weight function $w_{actual,P}$ which can be computed from the following ``local'' data, involving only information at each shape $\beta_j$:
\begin{enumerate}
    \item If $j > 0$, for each vertex in $V(\beta_{j})$, does this vertex appear in $\beta_{j'}$ for some $j' < j$? Note that the answer is automatically yes for the vertex in $U_{\beta_j}$.
    \item If $j < k+1$, for each vertex in $V(\beta_{j})$, does this vertex appear in $\beta_{j'}$ for some $j' > j$? Note that the answer is automatically yes for the vertex in $V_{\beta_j}$ if $j > 0$ and for the circle vertex/loose end in $\beta_0$.
    \item If there is a ``right-critical'' edge in $E(\beta_j)$ (defined below), does it vanish?
\end{enumerate}
For each $j$ and each $v \in V(\beta_j)$, we upper bound $w_{ideal,P}(v)$ based on this local data. In particular, if a vertex is incident to an edge which cannot vanish based on the local data at $\beta_j$, then we know it cannot be isolated and has a weight of $\sqrt{d}$ or $\sqrt{n}$. For $j = 0$, we can also assign weight $\sqrt{d}$ for the vertices in $U_{\alpha_P} \cup V_{\alpha_P}$ since we know they cannot be isolated. For other vertices, we conservatively upper bound their weights $d$ or $n$. We now make this formal.

\begin{definition}
We say that an edge is \textbf{safe} for shape $\beta_j$ if the local data on $\beta_j$ imply that it does not vanish, i.e. it appears in $\alpha_P$ with a positive label.
\end{definition}
\begin{proposition}
\label{prop:safe}
If $e = \{u,v\}$ is an edge in $\beta_j$ such that both of the following hold
\begin{enumerate}
    \item Either $u$ does not appear in $\beta_{j'}$ for any $j' < j$ or $v$ does not appear in $\beta_{j'}$ for any $j' < j$.
    \item Either $u$ does not appear in $\beta_{j'}$ for any $j' > j$ or $v$ does not appear in $\beta_{j'}$ for any $j' > j$.
\end{enumerate}
then $e$ is safe for $\beta_j$.
\end{proposition}
\begin{definition}
\label{def:local_values}
For each vertex $v \in V(\beta_j)$, we define $b_j(v)$ so that 
\begin{enumerate}
    \item If $v$ is a square vertex which is incident to an edge which is safe \aw{defn of safe involves right-critical edges... do we just mean the condition from proposition above?} \pax{Yes} for $\beta_j$ then $b_j(v) = \sqrt{d}$.
    \item If $j = 0$ and $v \in U_{\alpha_P} \cup V_{\alpha_P}$ then $b_j(v) = \sqrt{d}$.
    \item For all other square vertices, $b_j(v) = d$.
    \item If $v$ is a circle vertex which is incident to an edge which is safe for $\beta_j$ then $b_j(v) = \sqrt{n}$.
    \item For all other circle vertices, $b_j(v) = n$. 
\end{enumerate}
\end{definition}
Using the above definition, a natural attempt for the weight function $w_{actual,P}$ is 
\begin{align} 
\label{eqn:local_weight}
w_{local,P}(\beta_j) = \big(\frac{1}{\sqrt{d}} \big)^{\mathcal{I}(\beta_j)}\cdot 
\prod_{v \in V(\beta_j)}{b_j(v)^{1 - \frac{1}{2} \I \{v \text{ appears in } \beta_{j'} \text{ for some } j' < j\} - \frac{1}{2} \I\{v \text{ appears in } \beta_{j'} \text{ for some } j' > j\}}}
\end{align} 
where 
\[
\mathcal{I}(\beta_j) = {\I\bigg\{j = 0 \text{ and } \, \beta_0 \in \{ \alpha_{A^*,1},  \alpha_{A^*,2},\alpha_{A^*,3} \}\bigg\}}. 
\]
In other words, we divide by $\sqrt{d}$ for $j = 0$ if $\beta_0$ is $\alpha_{A^{*},1}$, $\alpha_{A^{*},2}$, or $\alpha_{A^{*},3}$.

\subsection{New proof of Lemma~\ref{lemma:Astar-Delta-k-ones}}
In this section, we show that the local weight function $w_{local,P}$ from the previous section is sufficient to complete the proof of Lemma~\ref{lemma:Astar-Delta-k-ones}. It suffices to verify the following two conditions:
\begin{enumerate}
    \item If $\beta_{start}$ is any of $\alpha_{A^*,1}, \alpha_{A^*,2}, \alpha_{A^*,3}$ and $\beta_{end} = \alpha_{1_n}$, then $w_{local,P}(\beta_{start}) w_{local,P}(\beta_{end}) \leq \max(\sqrt{d}n^{3/4},n)$.
    
    \item For all $j \in [k]$, $|w_{local,P}(\beta_j)c(\beta_j)| \leq \frac{\sqrt{n}}{d}$.
\end{enumerate}
Given these two conditions and following the discussion in Section~\ref{sec:norm-bounds-via-weights}, we have the following bound with probability $1-\poly(n)^{-1}$:
\begin{align*}
\alpha^{-(k+1)} \norm{\calA^*(\Delta^k 1_n)}_{op}   &\leq \polylog (n)^{O(k)} \sum_{\beta_1,\ldots,\beta_k \in \{\alpha_i : i \in \calI\}}{\sum_{P \in \mathcal{P}_{\beta_{start},\beta_1,\ldots,\beta_k,\beta_{end}}}{{|c_P|}\left(\prod_{j=1}^{k}{|c(\beta_j)|}\right)\norm{M_{\alpha_P}}_{op}}} \\
    &\leq \polylog(n)^{O(k)} \left(\frac{\sqrt{n}}{d}\right)^{k}\max_{P \in \mathcal{P}_{\beta_{start},\beta_1,\ldots,\beta_k,\beta_{end}}}{|c_P| \cdot  w_{local,P}(\beta_{start}) \cdot w_{local,P}(\beta_{end}) }
    \\&\leq \polylog(n)^{O(k)} \left(\frac{\sqrt{n}}{d}\right)^{k} \cdot O\left( \frac{1}{d^2} \right) \cdot \max(\sqrt{d}n^{3/4},n).
\end{align*}
which completes the proof of Lemma~\ref{lemma:Astar-Delta-k-ones}.

We now verify the two conditions on the local weight function. For the first condition, note that $w_{local,P}(\beta_{end}) = w_{local,P}(\alpha_{1_n}) = \sqrt{n}$. To handle contribution from $\beta_{start}$, we enumerate the following cases:
\begin{itemize}
    \item \textbf{Case $\beta_{start} = \alpha_{A^*,1}$:} By Lemma~\ref{lem:min-vertex-sep}, at least one of the two edges in $\alpha_{A^*,1}$ are safe. Hence, $w_{local,P} (\alpha_{A^*,1}) \leq \frac{1}{\sqrt{d}} b_0(u) b_0(v) b_0(x)^{1/2} = \sqrt{d} n^{1/4}$. 
    \item \textbf{Case $\beta_{start} = \alpha_{A^*,2}$:} In this case, $w_{local,P} (\alpha_{A^*,2}) \leq \frac{1}{\sqrt{d}} b_0(u) b_0(x)^{1/2} = \sqrt{n}$.
    \item \textbf{Case $\beta_{start} = \alpha_{A^*,3}$:} By Lemma~\ref{lem:min-vertex-sep},the single edge in $\alpha_{A^*,3}$ is safe. Hence, $w_{local,P}(\alpha_{A^*,3}) \leq \frac{1}{\sqrt{d}} b_0(u) b_0(x)^{1/2} = n^{1/4}$.
\end{itemize}
This completes the proof that $w_{local,P}(\beta_{start}) w_{local,P}(\beta_{end}) \leq \max(\sqrt{d}n^{3/4},n)$.


For the second condition, we fix $j \in [k]$. For $\beta_j$, we introduce a decoration $\tau(y)$ on every vertex $y$ that summarizes some information about its identification pattern $P$. For a vertex $y \in \beta_j$, define:
\begin{itemize}
    \item $\tau(y) = L$ if $y$ appears in $\beta_{j'}$ for $j' < j$ and does not appear in any $\beta_{j''}$ for $j'' > j$

    \item $\tau(y) = R$ if $y$ appears in $\beta_{j'}$ for $j' > j$ and does not appear in any $\beta_{j''}$ for $j'' < j$

    \item $\tau(y) = LR$ if $y$ appears in $\beta_{j'}$ for $j' < j$ and also appears in some $\beta_{j''}$ for $j'' > j$

    \item $\tau(y) = \emptyset$ otherwise
\end{itemize}

Below, for each shape $\alpha_i$ for $i \in \mathcal{I}$, we consider all possibilities of the decorations of the vertices of $\alpha_i$, reducing the number of cases when possible by symmetry. The tables below handle the essential cases. In the tables below, we use the term `Any' to denote that a vertex may have any of the decorations described above. Also define for $ y \in \beta_j$: 
\begin{align}
    \label{eqn:bbar_def}
    \overline{b}_j(y)
    &= b_j(y)^{1 - \frac{1}{2} \I \{y \text{ appears in } \beta_{j'} \text{ for some } j' < j\} - \frac{1}{2} \I\{y \text{ appears in } \beta_{j'} \text{ for some } j' > j\}} \nonumber 
    \\&= b_j(y)^{1- \frac{1}{2} \I (\tau(y) = L) - \frac{1}{2} \I(\tau(y) = R)}.  
\end{align}
Recall that for $1 \leq j \leq k$ ,  $w_{local,P}(\beta_j)$ is the product of the $\overline{b}_j(y)$'s, see \eqref{eqn:local_weight}. We now analyze the possible cases for $\beta_j$:
\begin{itemize}
    \item \textbf{Case $\beta_j = \alpha_1$:} A priori, there are a total of $2^1 \cdot 2^4 \cdot 2^4 \cdot 2^1$ cases since $\tau(u) \in \{ L, LR \}, \tau(x_1), \tau(x_2) \in \{ \emptyset, L, R, LR\}$, and $\tau(v) \in \{ R, LR \}$. By symmetry, each case reduces to one considered in Table \ref{table:alpha1-casework}. Note that the first row of Table \ref{table:alpha1-casework} stands for $32$ different cases. For this row, we slightly abuse notation and use $b_j(y)$ to specify an upper bound on the value of $y \in \{u, x_1, x_2, v\} \subset \alpha_{1}$ for all of these $32$ cases. 
    
    By inspection of Table \ref{table:alpha1-casework} and using that $n = d^2/\polylog(d)$, we conclude that 
    \begin{align} 
    \label{eqn:alpha2a_local}
    w_{local,P}(\beta_j) = w_{local,P}(\alpha_{1}) 
    \leq d \sqrt{n}.  
    \end{align}
    Also note that $c(\beta_j) = c(\alpha_{1}) = O(1/d^2)$.
    
    \item \textbf{Case $\beta_j = \alpha_{2a}$:} A priori, there are a total of $2^1 \cdot 2^4 \cdot 2^1$ cases since $\tau(u) \in \{ L, LR \}, \tau(x) \in \{ \emptyset, L, R, LR\}$, and $\tau(v) \in \{ R, LR \}$. By symmetry, each case reduces to one considered in Table \ref{table:alpha2a-casework}. Note that the first row of Table \ref{table:alpha2a-casework} stands for $4$ different cases. For this row, we slightly abuse notation and use $b_j(y)$ to specify an upper bound on the value of $y \in \{u, x, v\} \subset  \alpha_{2a}$ for all of these $4$ cases. 
    
    By inspection of Table \ref{table:alpha2a-casework} and using that $n = d^2/\polylog(d)$, we conclude that 
    \begin{align} 
    \label{eqn:alpha2a_local}
    w_{local,P}(\beta_j) = w_{local,P}(\alpha_{2a}) 
    \leq n.  
    \end{align}
    Also note that $c(\beta_j) = c(\alpha_{2a}) = O(1/d^2)$.
    
    \item \textbf{Case $\beta_j = \alpha_{3a}$:} First, note that $w_{local,P}(\beta_j) = b_j(u)^0 \Bar{b}_j(x_1) \Bar{b}_j(x_2) = \Bar{b}_j(x_1) \Bar{b}_j(x_2)$ because $u$ is identified with vertices to the left and right of $\beta_j$. It is straightforward to enumerate the possible decorations of $x_1,x_2$ and verify that $\Bar{b}_j(x_1) \Bar{b}_j(x_2) \leq d$. Thus, $w_{local,P}(\alpha_{3a}) \leq d$. Also, recall that $|c(\beta_j)| = |c(\alpha_{3a})| = O(1/d^2)$.
    
    \item \textbf{Case $\beta_j = \alpha_{3b}$:} Recall that $\alpha_{3b}$ has $U_{\alpha_{3b}} = V_{\alpha_{3b}} = (u)$. By the rules for graph matrix multiplication (see Section \ref{sec:product_rules}), $u \in \alpha_{3b}$ is identified with a circle vertex in $\beta_{j-1}$ and $\beta_{j+1}$. Hence $\tau(u) = LR$. By Definition \ref{def:local_values} and \eqref{eqn:bbar_def}, we have $\overline{b}_j(u) = 1$. Moreover, $\overline{b}_j(x) \leq \sqrt{d}$. Therefore,
    \begin{align}
    \label{eqn:alpha3b_local}
    w_{local,P}(\beta_j)
    = w_{local,P}(\alpha_{3b}) \leq \sqrt{d} 
    \end{align}
    Also recall that $|c(\beta_j)| = |c(\alpha_{3b})| = O(1/d)$. 

    \item \textbf{Case $\beta_j = \alpha_4$:} The proof is very similar to the one for $\alpha_{3b}$. Since $U_{\alpha_{4}} = V_{\alpha_4} = (u)$, we see that $\tau(u) = LR$, so $\overline{b}_j(u) = 1$. And automatically, $\overline{b}_j(x) \leq \sqrt{d}$. Hence
    \begin{align}
    \label{eqn:alpha3b_local}
    w_{local,P}(\beta_j)
    = w_{local,P}(\alpha_{4}) \leq \sqrt{d} 
    \end{align}
    Also recall that $|c(\beta_j)| = |c(\alpha_{4}) |= O(1/d^2)$.
\end{itemize}


\begin{table}[h!]
\centering
\begin{tabular}{ c|c|c|c|c|c|c } 
 % \hline
 $\tau(u)$ & $\tau(x)$ & $\tau(v)$ & $\overline{b}_j(u)$ & $\overline{b}_j(x)$ & $\overline{b}_j(v)$ & Product \\ 
\hline
 LR & Any & LR & $1$ & $d$ & $1$ & $d$\\
 LR & R & R & $1$ & $d^{1/2}$ & $n^{1/2}$ & $n^{1/2} d^{1/2}$ \\ 
 LR &  $\emptyset$ & R & $1$ & $d^{1/2}$ & $n^{1/4}$ & $n^{1/4} d^{1/2}$ \\ 
 LR & L  & R & $1$ & $d^{1/4}$ & $n^{1/4}$ & $n^{1/4} d^{1/4}$ \\ 
 L & $\emptyset$ & R & $n^{1/4}$ & $d^{1/2}$ & $n^{1/4}$ & $n^{1/2} d^{1/2}$ \\ 
 L & L & R & $n^{1/2}$ & $d^{1/4}$ & $n^{1/4}$ & $n^{3/4} d^{1/4}$ \\
 L & LR & R & $n^{1/2}$ & $1$ & $n^{1/2}$ & $n$ \\
 % \hline
\end{tabular}
\caption{Case work for $\alpha_{2a}$.}
\label{table:alpha2a-casework}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{ c|c|c|c|c|c|c|c|c } 

 $\tau(u)$ & $\tau(x_1)$ & $\tau(x_2)$ & $\tau(v)$ & $\overline{b}_j(u)$ & $\overline{b}_j(x_1)$ & $\overline{b}_j(x_2)$ & $\overline{b}_j(v)$ & Product \\ 
 \hline
 LR & Any & Any & Any & $1$ & $d^{1/2}$ & $d^{1/2}$ & $n^{1/2}$ & $n^{1/2} d$ \\
 L & $\perp$ & $\perp$ & R & $n^{1/4}$ & $d^{1/2}$ & $d^{1/2}$ & $n^{1/4}$ & $n^{1/2}d$ \\
 L & $\perp$ & L & R & $n^{1/4}$ & $d^{1/2}$ & $d^{1/4}$ & $n^{1/4}$ & $n^{1/2} d^{3/4}$ \\
 L & $\perp$ & LR & R & $n^{1/4}$ & $d^{1/2}$ & $1$ & $n^{1/4}$ & $n^{1/2} d^{1/2}$ \\
 L & L & L & R & $n^{1/2}$ & $d^{1/4}$ & $d^{1/4}$ & $n^{1/4}$ & $n^{3/4} d^{1/2}$ \\
 L & L & R & R & $n^{1/4}$ & $d^{1/4}$ & $d^{1/4}$ & $n^{1/4}$ & $n^{1/2} d^{1/2}$ \\
 L & L & LR & R & $n^{1/2}$ & $d^{1/4}$ & $1$ & $n^{1/4}$ & $n^{3/4} d^{1/4}$ \\
 L & LR & LR & R & $n^{1/2}$ & $1$ & $1$ & $n^{1/2}$ & $n$ \\
 
\end{tabular}
\caption{Case work for $\alpha_1$.}
\label{table:alpha1-casework}
\end{table}


\subsection{The actual weighting scheme}
Unfortunately, while this local weight function is sufficient for proving Lemma~\ref{lemma:Astar-Delta-k-ones}, the bound it gives is too loose for terms arising in $\calA^* (\Delta^k w)$ and $1^T \Delta^k w$. Specifically, the above weighting scheme is too conservative when assigning weight to the vertices in $\alpha_w$ in the case that its single edge vanishes.

To handle this bad case, we decrease the weight on the square vertex of $\alpha_w$ when its edge vanishes. To compensate for this, we increase the weight on squares in other shapes. We then have to show that this increase is always sufficient to maintain the condition that $\prod_{j=0}^{k+1}{w_{actual,P}(\beta_{j})} \geq \prod_{j=0}^{k+1}{w_{ideal,P}(\beta_{j})}$. To describe the actual weighting scheme we use, we introduce the notion of \textit{critical edges}.


\begin{definition}
We define the following two types of edges to be \textbf{right-critical edges}:
\begin{enumerate}
    \item If the square vertex in $\alpha_w$ appears in $\beta_{j}$ for some $j < k+1$ then the edge in $\alpha_w$ is a right-critical edge.
    \item If $\beta_j = \alpha_{2a}$, the circle vertex $u$ in $U_{\beta_j}$ does not appear in $\beta_{j'}$ for any $j' > j$, the circle vertex in $V_{\beta_j}$ does not appear in $\beta_{j''}$ for any $j'' < j$, and the square vertex $x$ appears in $\beta_{j'''}$ and $\beta_{j''''}$ for some $j''' < j < j''''$ then the edge $\{u,x\}_2$ in $\beta_j = \alpha_{2a}$ is a right-critical edge.
\end{enumerate}
\end{definition}
\begin{definition}
We define a \textbf{left-critical edge} of $\beta_j$ to be an edge $e = \{u,v\}$ such that one of the following two cases holds:
\begin{enumerate}
    \item $l_e = 2$, $u$ appears in $\beta_{j'}$ for some $j' > j$, and $v$ appears in $\beta_{j''}$ for some $j'' > j$.
    \item $l_e = 1$, $u$ appears in $\beta_{j'}$ for some $j' > j$, $v$ appears in $\beta_{j''}$ for some $j'' > j$, $u$ appears in $\beta_{j'''}$ for some $j''' < j$, and $v$ appears in $\beta_{j''''}$ for some $j'''' < j$.
\end{enumerate}
\end{definition}
We now observe that if there is a vanishing right-critical edge then there must be another shape containing a left-critical edge but does not have a vanishing right-critical edge. We construct our actual weighting scheme so that all of the shapes which have a left-critical edge but no vanishing right-critical edge can compensate for the ``excess'' weight on the square of $\alpha_w$.
\begin{lemma}
Given an identification pattern $P$ on $\beta_{0},\beta_1,\ldots,\beta_{k},\beta_{k+1}$, if there is a $j \in [k+1]$ such that $\beta_j$ has a vanishing right-critical edge then there is a $j' < j$ such that $\beta_{j'}$ has a left-critical edge and does not have a vanishing right-critical edge.
\end{lemma}
\begin{proof}
We prove this lemma by induction on $j$. Assume the result is true for $j = m$ and assume that $\beta_{j}$ has a vanishing right-critical edge where $j = m+1$.

For both of the cases where there is a right-critical edge ($\alpha_w$ where the square appears earlier and $\alpha_{2a}$ where the square appears both earlier and later, the circle in $U$ does not appear later on and the circle in $V$ does not appear earlier), this edge cannot appear in $\beta_{j'}$ for any $j' > j$. Let $j'$ the largest index such that $j' < j$ and this edge appears in $\beta_{j'}$ (such an edge must exist as otherwise it would not vanish).

Observe that this edge $e$ must be a left-critical edge in $\beta_{j'}$. To see this, observe that $e$ appears in $\beta_{j}$ where $j > j'$ so if $l_e = 2$ then $e$ is automatically a left-critical edge. If $l_e = 1$ then $e$ must also appear in $\beta_{j''}$ for some $j'' < j'$ as otherwise $e$ cannot vanish (two parallel edges with labels $1$ and $2$ give a term with label $1$ and a term with label $3$ so they do not vanish). Thus, $e$ is a left-critical edge in this case as well.

If $\beta_{j'}$ does not have a vanishing right-critical edge then we are done. If $\beta_{j'}$ does have a vanishing right critical edge (in which case it must be $\alpha_{2a}$) then by the inductive hypothesis there is a $j'' < j'$ which has a left-critical edge but does not have a vanishing right-critical edge, as needed.
\end{proof}


\subsection{Paying for the Extra Square: completing the proof of Lemma}

\begin{lemma}
Let $x_{extra}$ be the square in $\alpha_w$. If $\beta_j$ has a left-critical edge and no vanishing right-critical edge then 
\[
w_{actual,P}(\beta_j)w_{actual,P}(x_{extra}) \geq w_{ideal,P}(\beta_j)w_{ideal,P}(x_{extra})
\]
\end{lemma}
\begin{proof}
There are several cases to consider. 
\begin{enumerate}
    \item If $\beta_j = \alpha_{2a}$, $\tau(x)$ is $R$ or $LR$, and the edge between $u$ and $x$ does not vanish then $w_{actual,P,j}(u) \leq \sqrt[4]{n}$, $w_{actual,P,j}(x) = \sqrt{d}$, and $w_{actual,P,j}(v) \leq \sqrt{n}$. Note that
    $w_{ideal,P}(x_{extra}) = \sqrt{d}$ (as this square cannot be isolated) so $w_{actual,P,j}(x) \geq w_{ideal,P}(x_{extra})$ and thus
    \[
        w_{actual,P}(\beta_j)w_{actual,P}(x_{extra}) \geq w_{ideal,P}(\beta_j)w_{ideal,P}(x_{extra})
    \]
    \item If $\beta_j = \alpha_{2a}$ and $\tau(u) = LR$ then $w_{actual,P,j}(u) = 1$, $w_{actual,P,j}(x) = d$, and $w_{actual,P,j}(v) \leq \sqrt{n}$ so $w_{actual,P,j}(x) \geq w_{ideal,P}(x_{extra})$ and thus 
    \[
    w_{actual,P}(\beta_j)w_{actual,P}(x_{extra}) \geq w_{ideal,P}(\beta_j)w_{ideal,P}(x_{extra})
    \]
    Similar logic applies if $\tau(x) = LR$.
    \item If $j = 0$ and $\beta_0 = \alpha_{A^{*},3}$ then $w_{ideal,P}(x_{extra}) = 1$ so we already have that $w_{actual,P,k+1}(x_{extra}) \geq w_{ideal,P}(x_{extra})$ 
    \item If $\beta_j = \alpha_1$ then we must have $\tau(u) = LR$ or $\tau(v) = LR$. If $\tau(u) = LR$, we have that 
    $w_{actual,P,j}(u) = 1$, $w_{actual,P,j}(x_1) = w_{actual,P,j}(x_2) = \sqrt{d}$, and $w_{actual,P,j}(v) \leq \sqrt{n}$.
    
    Let $i \in \{1,2\}$ be the index such that $x_i$ is identified with $x_{extra}$. We must also have that $\tau(x_i) = LR$ so $w_{ideal,P,j}(x_i) = 1$. This implies that $w_{actual,P,j}(x_i)w_{actual,P,k+1}(x_{extra}) = \sqrt{d} \geq w_{ideal,P,j}(x_i)w_{ideal,P,k+1}(x_{extra})$ which in turn implies that 
    \[
    w_{actual,P}(\beta_j)w_{actual,P}(x_{extra}) \geq w_{ideal,P}(\beta_j)w_{ideal,P}(x_{extra})
    \]
    \item If $\beta_j = \alpha_{3a}$ then $w_{actual,P}(x_1) = \sqrt{d}\sqrt[4]{n}$ and $w_{actual,P}(x_2) = \sqrt{d}\sqrt[4]{n}$
    so if $x_{extra}$ is $x_i$ for $i \in \{1,2\}$ then $w_{actual,P,j}(x_i)w_{actual,P,k+1}(x_{extra}) \geq d$.
    \item If $\beta_j = \alpha_{3b}$ then $w_{actual,P}(x) = \sqrt{d}\sqrt[4]{n}$ so $w_{actual,P,j}(x)w_{actual,P,k+1}(x_{extra}) \geq d$.
    \item If $\beta_j = \alpha_{4}$ then $w_{actual,P}(x) = \sqrt{d}\sqrt[4]{n}$ so $w_{actual,P,j}(x)w_{actual,P,k+1}(x_{extra}) \geq d$.
\end{enumerate}
\end{proof}


==> Notes/junk.tex <==
\subsection{Old proof of Lemma~\ref{lemma:Astar-Delta-k-ones}}



% {\pax{It seesec:local_weights}at technically we only need this proof for $k = 1$, since the truncation at $T = 2$ works for $\calA^* B^{-1} 1_n$ and we explicitly analyzed the $k = 0$ term. That being said, it may be helpful to include the full details as a warm-up for Lemmas \ref{lemma:1T-Delta-k-w} and \ref{lemma:Astar-Delta-k-w} ? If so let's just make that clear with a comment here. }}

\vspace{0.3cm}

\pax{I changed all $\calA^{*}$'s to $\calA^*$'s; let's reserve the former dagger notation for pseudoinverse.}

\begin{claim}
\label{claim:min-vertex-sep}
For all $k \in \mathbb{N} \cup \{0\}$, for any shape $\alpha$ arising in the graph matrix representation of $\calA^{*} (\Delta^k 1_n)$ or the graph matrix representation of $\calA^{*} (\Delta^k w)$, it holds that $U_\alpha$ and $V_\alpha$ each consist of one square vertex (possibly the same) and are connected by a path of edges in $E(\alpha)$. Hence, when $n \leq d^2$, the minimum weight vertex separator of $\alpha$ consists of the square in $U_\alpha$ (or $V_\alpha$). \aw{this is redundant since we've already proved this claim in higher generality?}
\end{claim}
\begin{proof}
To prove this, it is sufficient to prove the following lemma
\begin{lemma}\label{lem:Aadjointstructural}
For any shape $\alpha$ arising in the graph matrix representation of $\calA^{*} (\Delta^k 1_n)$ or the graph matrix representation of $\calA^{*} (\Delta^k w)$, either $U_{\alpha} = V_{\alpha} = (u)$ where $u$ is a square vertex or $U_{\alpha} = (u)$, $V_{\alpha} = (v)$ where $u$ and $v$ are distinct square vertices and $u$ and $v$ are the only vertices with odd degree.
\end{lemma}
With this lemma, the result follows easily. If $U_{\alpha} = V_{\alpha} = (u)$ then the result is trivial. If $U_{\alpha} = (u)$, $V_{\alpha} = (v)$ where $u$ and $v$ are distinct square vertices and are the only vertices with odd degree then $u$ and $v$ must be in the same connected component of $\alpha$ due to the following fact.
\begin{proposition}
For any undirected graph $G$, for any connected component $C$ of $G$, $\sum_{v \in C}{deg(v)}$ is even.
\end{proposition}
\begin{proof}
This is the handshaking lemma and can be proved by observing that $\sum_{v \in C}{deg(v)} = 2|E(C)|$ which is even.
\end{proof}
\begin{proof}[Proof of Lemma \ref{lem:Aadjointstructural}]
To prove Lemma \ref{lem:Aadjointstructural}, we consider what shapes $\alpha$ can arise. 
We start by defining the following shapes corresponding to $A^{*}$ and to $w$.

\pax{The notation `$w$' was way overloaded, so I changed the name of an interior vertex in a shape to be called `$x$' instead.}

% \pax{Below needs to be defined before Section \ref{sec:normbound_strat}}
% \begin{definition}
% We define $\alpha_{A^{*},1}$, $\alpha_{A^{*},2}$, and $\alpha_{A^{*},3}$ to be the shapes such that 
% \begin{enumerate}
%     \item $U_{\alpha_{A^{*},1}} = (u)$ and  $V_{\alpha_{A^{*},1}} = (v)$ where $u, v$ are square vertices, $W_{\alpha_{A^{*},1}} = \{x\}$ where $x$ is a circle vertex, and $E(\alpha_{A^{*},1}) = \{\{u,x\}, \{x,v\}\}$.
%     \item $U_{\alpha_{A^{*},2}} = V_{\alpha_{A^{*},2}} = (u)$ where $u$ is a square vertex, $W_{\alpha_{A^{*},2}} = \{x\}$ where $x$ is a circle vertex, and $E(\alpha_{A^{*},2}) = \emptyset$.
%     \item $U_{\alpha_{A^{*},3}} = V_{\alpha_{A^{*},3}} = (u)$ where $u$ is a square vertex, $W_{\alpha_{A^{*},3}} = \{x\}$ where $x$ is a circle vertex, and $E(\alpha_{A^{*},3}) = \{\{u,x\}_2\}$.
% \end{enumerate}
% Recall that $\alpha_{w}$ is the shape such that 
% $U_{\alpha_{w}} = (u)$ and $V_{\alpha_{w}} = \emptyset$ where $u$ is a circle vertex, $W_{\alpha_{w}} = \{x\}$ where $x$ is a square vertex, and $E(\alpha_{w}) = \{\{u,x\}_2\}$.
% \end{definition}
% Insert pictures here.

Observe that any shape $\alpha$ arising in the graph matrix representation of $\calA^* (\Delta^k 1_n)$ or the graph matrix representation of $\calA^* (\Delta^k w)$ can be obtained using the following sequence of operations.

We start with either $\alpha_{A^{*},1}$, $\alpha_{A^{*},2}$, or $\alpha_{A^{*},3}$. In all three cases, we call the vertex $x$ in the corresponding shape to be the (initial) \textit{loose end}. 



We now do the following $k$ times.
\begin{enumerate}
    \item Append one of the shapes $\alpha_i$ in $\Delta$ by gluing $U_{\alpha_i} = (u)$ to the current loose end and making $V_{\alpha_i} = (v)$ the new loose end.
    \item For each vertex in $V(\alpha_i) \setminus U_{\alpha_i}$, either leave it alone or identify it with an existing vertex of the same type (circle or square) which is not $u$ and has not yet been merged with a vertex in $V(\alpha_i) \setminus U_{\alpha_i}$.
    \item Whenever we have two parallel labeled edges, replace them with a single labeled edge. The parity of the resulting label will be the same as the parity of the sum of the original labels.
\end{enumerate}
For shapes arising from $\calA^{*} (\Delta^k 1_n)$, we stop here (tying up the loose end). For shapes arising from $\calA^{*} (\Delta^k w)$, we append $\alpha_w$ to the existing shape by gluing $U_{\alpha_w} = (u)$ to the current loose end (which ties up the loose end). Letting $V_{\alpha_w} = (v)$, we then either leave $v$ alone or merge it with an existing vertex which is not $u$. If this creates two parallel labeled edges, we replace them with a single labeled edge.

We now make the following observations
\begin{enumerate}
    \item For all of the shapes in $\Delta$, all of the vertices have even degree.
    \item Whenever two vertices are glued together or merged, the parity of the degree of the resulting vertex is equal to the parity of the sum of the degrees of the original vertices.

    \pax{Do `gluing together' and `merging' mean the same thing? If so, let's just use one word for this. I think `identifying' is clear since we wanted to define an `identification scheme.' }
    
    \item No other operation affects the parities of the degrees of the vertices.
\end{enumerate}
Letting $U_{\alpha} = (u)$ and $V_{\alpha} = (v)$, these observations imply that either $u = v$ or $u$ and $v$ are the only vertices with odd degree. 
\end{proof} 

\begin{claim}
For all $i,j \in \mathbb{N}$, if we decompose ${h_i}{h_j}$ as ${h_i}{h_j} = \sum_{k}{c_{ijk}h_k}$ then we will have that $c_{ijk} = 0$ unless $k$ has the same parity as $i+j$ and $|j-i| \leq k \leq i + j$.
\end{claim}

\pax{This claim is a bit out of place and it's not very clear where it was used in the proof above. Also does this claim need proof?} 

\end{proof}

\begin{proof}[Proof of Lemma~\ref{lemma:Astar-Delta-k-ones}]
As illustrated in Section~\ref{sec:shapes}, $-\Delta = B - \alpha I_n$ admits the following graph matrix representation
\[
\sum_{i \in \calI} \lambda_{\alpha_i} M_{\alpha_i}.
\]
Plugging this into $\calA^*(\Delta^k 1_n)$, multiplying the terms out and applying the triangle inequality yields: 

\[
\norm{\calA^*(\Delta^k 1_n)}_{op} \leq |\calI|^k \max_{(i_1, \ldots, i_k) \in \calI^k} \norm{\calA^* \left( \prod_{j \in [k]} \lambda_{\alpha_{i_j}} M_{\alpha_{i_j}} 1_n \right)}_{op} .
\]
In the following, fix any $(i_1, \ldots, i_k) \in \calI^k$. By the multiplication rule (Definition~\ref{defn:mult-rule}), $\calA^* \left( \prod_{j \in [k]} \lambda_{\alpha_{i_j}} M_{\alpha_{i_j}} 1_n \right)$ admits a graph matrix representation as a sum of shapes; we denote the set of such shapes by $S$. Note that any $\alpha \in S$ contains at most $4k + 3$ vertices and at most $4k+3$ edges and has the property that $U_\alpha$ and $V_\alpha$ both contain one square vertex -- note that the square vertex in $U_\alpha$ and $V_\alpha$ may be identified. Hence, by Proposition~\ref{prop:number-of-shapes-bound} , $|S| = k^{O(k)}$. We will now fix one such $\alpha \in S$ and derive a high-probability bound $\mathcal{B}$  on $\norm{\lambda_\alpha M_\alpha}_{op}$. Having done so, we can apply the union bound and the triangle inequality to conclude that with high probability:


\[
\alpha^{-(k+1)} \norm{\calA^* (\Delta^k 1_n)}_{op} \leq \alpha^{-(k+1)} |\calI|^k \cdot |S| \cdot \mathcal{B} = \alpha^{-(k+1)} k^{O(k)} \cdot \mathcal{B}.
\]

Note that we overload notation, and in the equation above $\alpha \sim d^2$ is a scalar. \aw{statement of this lemma doesn't involve the scalar $\alpha$, so we shouldn't need it here?}

Next, we observe that the shape $\alpha$ is realized from the product of $k+2$ shapes. The first shape is either $\alpha_{A1}$ or $\alpha_{A2}$, coming from $\calA^*$. The next $k$ shapes are each of the form $\alpha_i$ for some $i \in \calI$, coming from $\Delta^k$. The final shape is the trivial shape of the vector $1_n$. By Claim~\ref{claim:min-vertex-sep}, the minimum weight vertex separator of $\alpha$ is just the square vertex in $U_\alpha$ (which comes from a square vertex in either $\alpha_{A1}$ or $\alpha_{A2}$).  Given this, it remains to define a faithful weighting scheme and calculate the associated norm bound it gives on $\lambda_\alpha M_\alpha$. \pax{Need to define what faithful means here and also explain the intuition behind the weighting scheme. ie, we have some graph matrix norm bounds that depend on the true weights, we find some convenient way to upper bound these weights, etc...}

\TODO{Make some definitions so that the following makes sense}
To define the weighting scheme, we need to assign a weight to each vertex $v$ in each of the $k+2$ shapes $\sigma$ from whose product $\alpha$ is realized. For each such $v$ in each such $\sigma$, we define the weight of $v$ as follows: \pax{$v$ here means any vertex of $\sigma$, or just the rightmost one?}
\begin{itemize}
    \item If $v$ is not identified with any vertex to its left or not identified with any vertex to its right (i.e. it is either the left-most or right-most occurrence) then:
        \begin{itemize}
            \item If we can determine that $v$ cannot be isolated in $\alpha$ by looking only at $\sigma$ and its identification pattern, then assign $v$ weight $d^{1/4}$ if it is a square and $n^{1/4}$ if it is a circle.

            \pax{What are the rules for determining if $v$ can be isolated or not?} 
            
            \item Otherwise, assign $v$ weight $d^{1/2}$ if it is a square and $n^{1/2}$ if it is a circle.
        \end{itemize}
    \item Otherwise, assign $v$ weight 1.
\end{itemize}
By construction, this weighting scheme is faithful. It remains to calculate the associated norm bound it gives on $M_\alpha$. Note that the norm bound is simply the product of weights of the $k+2$ shapes; we now calculate the the weights of each of these shapes. \TODO{Define what weight of a shape means.}
\begin{itemize}
    \item \textbf{First shape:} This shape comes from $\calA^*$; it is either $\alpha_{A1}$ or $\alpha_{A2}$. We show that the weight is at most $\max (\sqrt{n}, \sqrt{d}n^{1/4})$.
        \begin{itemize}
            \item \textbf{Case A1:} If the shape is $\alpha_{A1}$, then the weight is $\sqrt{d}n^{1/4}$. 
            To see this, first note that the minimum weight vertex separator is $v_1$, so the remaining square vertex $v_2$ can contribute at most $\sqrt{d}$ weight. By Claim~\ref{claim:min-vertex-sep} the single circle vertex $u$ is not isolated (since that would imply $v_1, v_2$ could be disconnected), so it contributes weight at most $n^{1/4}$.
            \item \textbf{Case A2:} If the shape is $\alpha_{A2}$, then because the minimum weight vertex separator is its remaining square, only the single remaining circle vertex can contribute to the weight. This vertex has weight at most $\sqrt{n}$.
        \end{itemize} 
    \item \textbf{Middle $k$ shapes:} These shapes are each of the form $\alpha_i$ for some $i \in \calI$. We enumerate these possible cases and show that the weight of any such term is at most $O(\max (\sqrt{n}d,n^{3/4}\sqrt{d})$. \aw{only list larger term? would help keep things simpler}  With the exception of $\alpha_{}3b$, all shapes below have a coefficient of $O(1)$.
        \begin{itemize}
            \item \textbf{Case 1:} If the shape is $\alpha_1$, then the weight is at most $O(\max (\sqrt{n}d,n^{3/4}\sqrt{d}))$. We compute this bound by enumerating all the possible intersection patterns for the vertices in $\alpha_1$; see Table~\ref{table:alpha1-casework}. There are actually 64 possible patterns, but by symmetry of the shape $\alpha_1$, we only need to analyze those patterns listed in the table.
            \item \textbf{Case 2a:} If the shape is $\alpha_{2a}$, then the weight is at most $O(\max (\sqrt{nd},n^{3/4}d^{1/4}))$. We compute this bound by enumerating all the possible intersection patterns for the vertices in $\alpha_{2a}$; see Table~\ref{table:alpha2a-casework}. There are actually 16 possible patterns, but by symmetry of the shape $\alpha_{2a}$, we only need to analyze those patterns listed in the table.
            \item \textbf{Case 3a:} If the shape is $\alpha_{3a}$, then the weight is at most $O(d)$. To see this, note that $u$ always gets assigned weight 1 and $x_1, x_2$ get assigned weight at most $\sqrt{d}$ each. 
            \item \textbf{Case 3b:}
            If the shape is $\alpha_{3b}$, then the weight is at most $O(d^{3/2})$. To see this, note that $u$ always gets assigned weight 1 and $x$ gets assigned weight at most $\sqrt{d}$ and that the coefficient associated with this shape is $O(d)$.
            \item \textbf{Case 4:} If the shape is $\alpha_{4}$, then the weight is at most $\sqrt{d}$. To see this, note that $u$ always gets assigned weight 1 and $x$ gets assigned weight at most $\sqrt{d}$.
        \end{itemize}
    \item \textbf{Last shape:} The last shape corresponds to $1_n$; it contains a single vertex so its weight is at most $\sqrt{n}$.
\end{itemize}

\begin{table}[h!]
\centering
\begin{tabular}{ |c|c|c|c|c|c|c|c|c| } 
 \hline
 $u$ & $x_1$ & $x_2$ & $v$ & $w(u)$ & $w(x_1)$ & $w(x_2)$ & $w(v)$ & Product \\ 
 \hline
 LR & Any & Any & Any & $1$ & $d^{1/2}$ & $d^{1/2}$ & $n^{1/2}$ & $n^{1/2} d$ \\
 L & $\emptyset$ & $\emptyset$ & R & $n^{1/4}$ & $d^{1/4}$ & $d^{1/4}$ & $n^{1/4}$ & $n^{1/2} d^{1/2}$ \\
 L & $\emptyset$ & L & R & $n^{1/4}$ & $d^{1/4}$ & $d^{1/4}$ & $n^{1/4}$ & $n^{1/2} d^{1/2}$ \\
 L & $\emptyset$ & LR & R & $n^{1/4}$ & $d^{1/4}$ & $1$ & $n^{1/4}$ & $n^{1/2} d^{1/4}$ \\
 L & L & L & R & $n^{1/2}$ & $d^{1/4}$ & $d^{1/4}$ & $n^{1/4}$ & $n^{3/4} d^{1/2}$ \\
 L & L & R & R & $n^{1/4}$ & $d^{1/4}$ & $d^{1/4}$ & $n^{1/4}$ & $n^{1/2} d^{1/2}$ \\
 L & L & LR & R & $n^{1/2}$ & $d^{1/4}$ & $1$ & $n^{1/4}$ & $n^{3/4} d^{1/4}$ \\
 L & LR & LR & R & $n^{1/2}$ & $1$ & $1$ & $n^{1/2}$ & $n$ \\
 \hline
\end{tabular}
\caption{Case work for $\alpha_1$.}
%\label{table:alpha1-casework}
\end{table}


\pax{Here's what I got for Table 1 (last four rows are the same):} 




\begin{table}[h!]
\centering
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
 $u$ & $x$ & $v$ & $w(u)$ & $w(x)$ & $w(v)$ & Product \\ 
 \hline
 LR & Any & Any & $1$ & $d^{1/2}$ & $n^{1/2}$ & $n^{1/2} d^{1/2}$ \\ 
 L & $\emptyset$ & R & $n^{1/4}$ & $d^{1/4}$ & $n^{1/4}$ & $n^{1/2} d^{1/4}$ \\ 
 L & L & R & $n^{1/2}$ & $d^{1/4}$ & $n^{1/4}$ & $n^{3/4} d^{1/4}$ \\
 L & LR & R & $n^{1/2}$ & $1$ & $n^{1/2}$ & $n$ \\
 \hline
\end{tabular}
\caption{Case work for $\alpha_{2a}$.}
% \label{table:alpha2a-casework}/
\end{table}



\begin{table}[h!]
\centering
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
 $u$ & $x$ & $v$ & $w(u)$ & $w(x)$ & $w(v)$ & Product \\ 
\hline
 LR & Any & LR & $1$ & $d$ & $1$ & $d$\\
 LR & R & R & $1$ & $d^{1/2}$ & $n^{1/2}$ & $n^{1/2} d^{1/2}$ \\ 
 LR &  $\perp$ & R & $1$ & $d^{1/2}$ & $n^{1/4}$ & $n^{1/4} d^{1/2}$ \\ 
 LR & L  & R & $1$ & $d^{1/4}$ & $n^{1/4}$ & $n^{1/4} d^{1/4}$ \\ 
 L & $\perp$ & R & $n^{1/4}$ & $d^{1/2}$ & $n^{1/4}$ & $n^{1/2} d^{1/2}$ \\ 
 L & L & R & $n^{1/2}$ & $d^{1/4}$ & $n^{1/4}$ & $n^{3/4} d^{1/4}$ \\
 L & LR & R & $n^{1/2}$ & $1$ & $n^{1/2}$ & $n$ \\
 \hline
\end{tabular}
\caption{Case work for $\alpha_{2a}$.}
% \label{table:alpha2a-casework}
\end{table}



Hence, we may conclude by Theorem~\ref{thm:graph-matrix-norm-bound} that for any $\alpha \in S$, with probability $1- \epsilon$, 
\[
\norm{\lambda_\alpha M_\alpha}_{op} = \left( k \log(k) + \log (4n) + \log(1/\epsilon) \right)^{O(k)} \cdot \max (n,\sqrt{d}n^{3/4}) \cdot O(\max (\sqrt{n}d,n^{3/4}\sqrt{d}))^k
\]
Setting $\epsilon = \epsilon' /|\calI|^k |S|$ and using the fact that $|\calI|^k |S| = k^{O(k)}$, applying the union bound and triangle inequality gives that with probability $1-\epsilon'$,
\[
\norm{\calA^*(\Delta^k 1_n)}_{op} \leq \left( k \log(k) + \log (4n) + \log(1/\epsilon') \right)^{O(k)} \cdot \max (n,\sqrt{d}n^{3/4}) \cdot O(\max (\sqrt{n}d,n^{3/4}\sqrt{d}))^k
\]
\end{proof}

\pax{Above is what I got for Table \ref{table:alpha2a-casework}. Last two rows are the same. I had to expand out the first row a bit but still seems like there's a fair amount of slack for this shape. }

\subsection{Proof of Lemma~\ref{lemma:Astar-Binv-w} \aw{just Lemma~\ref{lemma:Astar-Delta-k-w}?}}
The proof follows that of Lemma~\ref{lemma:Astar-Binv-1} closely, but requires some modification to achieve the claimed norm bound. We first explain why the proof of Lemma~\ref{lemma:Astar-Binv-1}, without modification, gives a norm bound that is (multiplicatively) $\Tilde{O}(\sqrt{d})$ larger than the claimed bound. Then, we explain how to modify the weighting scheme to remove this extra factor.

Suppose we apply the same weighting scheme as in the proof of Lemma~\ref{lemma:Astar-Binv-1}. The only new shape that arises is the last shape, which now comes  from $w$ instead $1_n$. In the proof of Lemma~\ref{lemma:Astar-Binv-1}, $1_n$ contributes a weight of $\sqrt{n}$. \TODO{i use $\alpha_w$ to denote shape of $w$} Here, if the identification pattern for $\alpha_w$ is such that its edge does not vanish, then neither the square nor circle in $\alpha_w$ can be isolated, so the weight of $\alpha_w$ is $n^{1/4} d^{1/4} \leq \sqrt{n}$ when $n \geq d$. Hence, under the assumption that the edge of $\alpha_w$ does not vanish, the final norm bound is no bigger than the claimed bound.

So, it suffices to analyze the problematic case that the identification pattern for $\alpha_w$ is such that its edge vanishes. In this case, the square and circle in $\alpha_w$ are identified with some other square and circle, also connected by an edge with label 2, in a shape $\sigma$ from $\calA^*$ (either $\alpha_{A1}$ or $\alpha_{A2}$) or one of the middle $k$ shapes (one of $\alpha_i$ for $i \in \calI$). Both the circle and square of $\alpha_w$ may become isolated, so they are assigned weights $\sqrt{n}$ and $\sqrt{d}$, respectively. To complete the proof, we now enumerate the 7 possible cases for $\sigma$ and show that the weight of $\sigma$ can be always be adjusted so that the total weight of $\sigma$ and $\alpha_w$ is at most $\Tilde{O}(\max (n, n^{3/4} \sqrt{d}, d\sqrt{n}, d^2) \cdot \sqrt{n})$. Observe that if this holds, then the claimed norm bound holds. 

\begin{itemize}
    \item \textbf{Case A1:}
    \item \textbf{Case A2:}
    \item \textbf{Case 1:} \TODO{Slide 13 of Jamboard here}
    \item \textbf{Case 2a:} As shown in the first two rows of Table~\ref{table:alpha2a-casework}, total the weight of $\alpha_w$ (which contributes $\sqrt{dn}$ and $\alpha_{2a}$ (which contributes at most $\sqrt{dn}$) in either of these cases is at most $dn$. We now show how to analyze the remaining cases for the possible intersection patterns of $\alpha_{2a}$, corresponding to the final two rows of Table~\ref{table:alpha2a-casework}:
    \begin{itemize}
        \item \textbf{Case (L,R,R):} First, the circle vertex $u$ of $\alpha_{2a}$ cannot be isolated and is identified with a vertex from a shape to the left of $\alpha_{2a}$, so it has weight $n^{1/4}$. Next, the middle square vertex $w$ of $\alpha_{2a}$, which gets identified with the square vertex of $\alpha_w$, cannot be isolated but may not be identified with another vertex from a shape (not $\alpha_w$) to the right of $\alpha_{2a}$, so it has weight $d^{1/2}$. Finally, the circle vertex $v$ of $\alpha_{2a}$, which gets identified with the circle vertex of $\alpha_w$, can be isolated and may not be identified with another vertex from a shape (not $\alpha_w$) to the right of $\alpha_{2a}$, so it has weight $n$ Altogether, the total weight of $\alpha_{2a}$ and $\alpha_w$ is at most $n^{5/4} \sqrt{d}$.
        \item \textbf{Case (L,LR,R):} In this case, the square vertex of $\alpha_w$ gets identified with the square vertex $w$ of $\alpha_{2a}$ and the circle vertex of $\alpha_w$ gets identified with the circle vertex  $v$ of $\alpha_{2a}$. The circle vertex $u$ of $\alpha_{2a}$ is identified with a vertex in a shape to the left of $\alpha_{2a}$, so it has weight $n^{1/2}$. Next, the common square vertex of $\alpha_w$ and $\alpha_{2a}$ is identified with some square vertex in a shape to the left of $\alpha_{2a}$, so it has weight $d^{1/2}$. Finally, the common circle vertex of $\alpha_w$ and $\alpha_{2a}$ has weight $\sqrt{n}$ because it could be isolated and may not be identified with any other vertex to the left or right. Altogether, the weight of $\alpha_{2a}$ and $\alpha_w$ is $n \sqrt{d}$.
    \end{itemize}
    \item \textbf{Cases 3a, 3b, 4:} These shapes have a weight of $O(d^{3/2})$ each to begin with. So, the total weight of $\sigma$ and $\alpha_{2w}$ is $O(d^2 \sqrt{n})$.
\end{itemize}

\begin{theorem}[Corollary 5.49 of \cite{aubrun2017alice}]
\label{thm:gaussian-poly-conc}
Let $Z \sim \calN(0,I_n)$ and $X = Q(Z_1, \ldots, Z_n)$, where $Q: \R^n \rightarrow \R$ is a polynomial of degree at most $k$. Then for any $t \geq (2e)^{k/2}$,
\[
\Prob \left(|X - \E X| > t \sqrt{\Var (X)} \right) \leq \exp \left(- \frac{k}{2e} t^{2/k} \right).
\]
\end{theorem}



\subsection{Supporting technical lemmas for Lemma~\ref{lemma:weak-delta-bound}}
\label{sec:technical-lemmas}

\begin{theorem}[modified version of Theorem 5.62 of \cite{vershynin2010introduction}]
\label{thm:vershynin-562}
Let $A \in \R^{N \times n}$ ($N \geq n$) whose columns $A_j$ are independent isotropic random vectors in $\R^N$. Consider the incoherence parameter 
\[
m = \frac{1}{N} \E \max_{i \in [n]} \sum_{j \in [n] \setminus i} \ip{A_i}{A_j}^2.
\]
Then 
\[
\E \norm{\frac{1}{N}A^T A - I} \leq \frac{C}{N} \left( \sqrt{N n \log n} \cdot \E \max_{i \in [n]} \sqrt{1+\epsilon_i} +  \sqrt{N m \log n} \right)+ C \cdot \E \max_{i \in [n]} |\epsilon_i|,
\]
where $\norm{A_i}_2^2 = (1+\epsilon_i) N$ and $C$ is some absolute constant.
\end{theorem}
\begin{proof}
The proof is almost identical to that of Theorem 5.63 of~\cite{vershynin2010introduction}, but we reproduce it here for completeness. To begin, we require a rough a priori bound on $\norm{A}$. By Theorem 5.45 of \cite{vershynin2010introduction} since $A^T$ has independent isotropic random rows, we obtain
\[
\E \norm{A} = \E \norm{A^T} \leq \sqrt{n} + C_0 \sqrt{N \log n} \E_{A_T} \max_{i \in [n]} \sqrt{1 + \epsilon_i}.
\]

Next, by Lemma 5.63 of \cite{vershynin2010introduction} and some straightforward manipulations, we have that
\[
\E \norm{\frac{1}{N} A^TA - I_n} \leq \E \max_{i \in [n]}|\epsilon_i| + \frac{4}{N} \max_{T \subseteq [n]} \E \norm{\Gamma(T)},
\]
where $\Gamma (T) = (A_{T})^T A_{T^c}$. 
Note that conditioned on $A_{T^c}$, the rows of $\Gamma(T)$ are independent. By Theorem 5.48 and Remark 5.49 of \cite{vershynin2010introduction}, we then have
\[
\E_{A_T} \norm{\Gamma(T)} \leq \norm{\Sigma}^{1/2} \sqrt{|T|} + C_1 \sqrt{\log \min (|T|, |T^c|)} \sqrt{\E \max_{i \in T} \norm{\Gamma(T)_i}_2^2},
\]
where $\Gamma(T)_i$ is the $i^{th}$ row of $\Gamma(T)$, $\Sigma = \frac{1}{|T|} \sum_{i \in T} \Sigma_i$ and $\Sigma_i = \E_{A_T} \Gamma(T)_i \Gamma(T)_i^T$. Next, it can be verified, using the fact that the $A_i$ have mean zero and identity covariance that
\[
\norm{\Sigma} \leq \max_{i \in T} \norm{\E_{A_T} \Gamma(T)_i \Gamma(T)_i^T} \leq \norm{A_{T^c}}^2.
\]
Putting these pieces together, we have
\begin{align*}
\E \norm{\frac{1}{N} A^TA - I_n} &\leq \E \max_{i \in [n]}|\epsilon_i| + \frac{4}{N} \max_{T \subseteq [n]} \E \norm{\Gamma(T)} \\
&\leq \E \max_{i \in [n]}|\epsilon_i| + \frac{4}{N} \max_{T \subseteq [n]} \E_{A_{T^c}} \left( \norm{A_{T^c}} \sqrt{|T|} + C_1 \sqrt{\log \min (|T|, |T^c|)} \sqrt{\E_{A_T} \max_{i \in T} \norm{\Gamma(T)_i}_2^2} \right) \\
&\leq \E \max_{i \in [n]}|\epsilon_i| + \frac{4}{N} \max_{T \subseteq [n]} \left( \E \norm{A} \sqrt{n} + C_1 \sqrt{\log n} \sqrt{\E \max_{i \in T} \norm{\Gamma(T)_i}_2^2} \right) \\
&= \E \max_{i \in [n]}|\epsilon_i| + \frac{4}{N} \max_{T \subseteq [n]} \left( \E \norm{A} \sqrt{n} + C_1 \sqrt{\log n} \sqrt{\E \max_{i \in T} \sum_{j \in T^c} \ip{A_i}{A_j}^2} \right)\\
&\leq \E \max_{i \in [n]}|\epsilon_i| + \frac{4}{N} \left( \E \norm{A} \sqrt{n} + C_1 \sqrt{N m \log n} \right).
\end{align*}
The proof is complete by plugging in the a priori estimate on $\E \norm{A}$ into the final line above.
\end{proof}

\begin{proof}[Proof of Claim~\ref{claim:m-parameter-bound}]
Define the random variables $Z_j = \sum_{k \neq j}  \ip{\offdiag(u_j)}{\offdiag(u_k)}^2$ for $j \in [n]$ and the parameter $T = O(nd^2 \log^5 (nd^2))$ large enough. We have
\begin{align*}
m &= \frac{1}{N} \E \max_{j \in [n]} Z_j \\
&= \frac{1}{N} \int_{0}^\infty \Prob(\max_{j \in [n]} Z_j > t) dt \\
&= \frac{1}{N} \left( \int_{0}^T \Prob(\max_{j \in [n]} Z_j > t) dt + \int_{T}^\infty \Prob(\max_{j \in [n]} Z_j > t) dt \right) \\
&\leq \frac{T}{N} + \frac{n}{N} \int_{T}^\infty \Prob(Z_1 > t) dt.
\end{align*}
We now upper bound the tail probabilities. Note that $\E Z_1 = (n-1)d(d-1)$ and $\Var(Z_1) = O(n^2 d^4)$. Since $t \geq T$, we have that
\[
\Prob(Z_1 > t) = \Prob(Z_1 - \E Z_1 > t - \E Z_1) \leq \Prob(Z_1 - \E Z_1 > 0.99t).
\]
By Theorem~\ref{thm:gaussian-poly-conc}, for the degree-8 polynomial $Z_1$ in i.i.d.\ Gaussians, there is some constant $c > 0$ such that for all $t \geq T$,
\[
\Prob(Z_1 - \E Z_1 > 0.99t) \leq \exp\left(-c \frac{t^{1/4}}{n^{1/4} d^{1/2}}\right).
\]
Substituting this expression into the integral above and using $t \geq T$, we may conclude that the integral is $O(1)$.
\end{proof}

\begin{proof}[Proof of Claim~\ref{claim:eps-bound}]
Let $T = C d^{3/2} \log d$ for some constant $C > 0$ to be determined later. We have the following:
\begin{align*}
\frac{1}{N} \E N \cdot \max_{i \in [n]} | \epsilon_i | &= \frac{1}{N} \int_{0}^\infty \Prob (N \cdot \max_{i \in [n]} | \epsilon_i | > t) dt \\
&= \frac{1}{N}\int_{0}^T \Prob (N \cdot \max_{i \in [n]} | \epsilon_i | > t) dt + \frac{1}{N}\int_{T}^\infty \Prob (N \cdot \max_{i \in [n]} | \epsilon_i | > t) dt \\
&\leq \frac{T}{N} + \frac{n}{N} \int_{T}^\infty \Prob (N \cdot |\epsilon_1| > t) dt \\
&= \frac{T}{N} + \frac{n}{N} \int_{T}^\infty \Prob \left(|Y - \E Y| > t \right) dt,
\end{align*}
where $Y = \frac{1}{2}\left( \sum_{j=1}^d g_j^2 \right)^2 - \frac{1}{2} \sum_{j=1}^d g_j^4$ and $g \sim \calN(0, I_d)$. The proof is complete by showing that the integral is $O(1)$. Let $X =  \sum_{j=1}^d g_j^2$. We proceed by upper bounding the tail probability as follows: 
\[
\Prob \left(|Y - \E Y| > t \right) \leq \Prob \left( \left|\frac{1}{2} X^2 - \frac{d^2 +d}{2}\right| > t/2 \right) + \Prob \left(\left|\frac{1}{2} \sum_{j=1}^d g_j^4 - \frac{3d}{2}\right| > t/2 \right). 
\]
The second tail probability can be upper bounded by $2 \exp (- \Omega(\min (t^2/d, \sqrt{t})))$. For the first tail probability, we may write $X = d + \Delta$, where $\Delta = X - \E X$ and substitute to obtain
\begin{align*}
\Prob \left( \left|\frac{1}{2} X^2 - \frac{d^2 +d}{2}\right| > t/2 \right) &= \Prob \left( \left|\frac{1}{2} (X^2 -  \E X^2) \right| > t/2 \right)  \\
&= \Prob \left( \left|2d \Delta + \Delta^2 - \E \Delta^2 \right| > t \right) \\
&\leq \Prob \left( \left|2d \Delta \right| > \frac{1}{2} (t - \E \Delta^2) \right) + \Prob \left( \left| \Delta \right| > \sqrt{\frac{(t - \E \Delta^2)}{2}} \right). 
\end{align*}
Using the fact that $\E \Delta^2 = 2d$, the first probability above is at most $2 \exp(- \Omega (\min (t^2/d^3, t/d)))$ and the second probability is at most $2 \exp (- \Omega(\min(t/d, \sqrt{t})))$. After plugging these tail probabilities back into the original integral, it is straightforward to verify the integral is bounded by $O(1)$.
\end{proof}

\section{Graph Matrix Representation of $A^{*}A$ and $\Delta$}
For the purposes of computing ${\calA}{\calA}^{*}$, we can view $\calA$ as an $n \times d^2$ matrix $A$ with rows indexed by a single index in $[n]$ and columns indexed by either an ordered pair of indices in $[d]$ or a single index in $[d]$. With this view, we can decompose $A$ as $A = M_{\alpha_{A1}} + M_{\alpha_{A2}}$ and $A^{*} = M_{\alpha_{A1}}^T + M_{\alpha_{A2}}^T$ for the following shapes $\alpha_{A1}$ and $\alpha_{A2}$ (note that $\alpha_2$ is improper):
\begin{enumerate}
    \item $U_{\alpha_{A1}} = (u)$ where $u$ is a circle vertex, $V_{\alpha_{A1}} = (v_1,v_2)$ where $v_1,v_2$ are square vertices, $W_{\alpha_{A1}} = \{\}$ and $E(\alpha_{A1}) = \{\{u,v_1\}, \{u,v_2\}\}$.
    \item $U_{\alpha_{A2}} = (u)$ where $u$ is a circle vertex, $V_{\alpha_{A2}} = (v)$ where $v$ is a square vertex, $W_{\alpha_{A2}} = \{\}$ and $E(\alpha_{A2}) = \{\{u,v\}, \{u,v\}\}$.
\end{enumerate}
Insert picture here.

Multiplying $A$ and $A^{*}$, we have the following decomposition for ${\calA}{\calA}^{*} = {A}A^{*}$.
\[
{\calA}{\calA}^{*} = M_{\alpha_1} + M_{\alpha_2} + M_{\alpha_3} + M_{\alpha_4}
\]
where $\alpha_1$, $\alpha_2$, $\alpha_3$, and $\alpha_4$ are the following shapes (note that $\alpha_2$, $\alpha_3$, and $\alpha_4$ are improper):
\begin{enumerate}
    \item $U_{\alpha_{1}} = (u)$ and  $V_{\alpha_{1}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{1}} = \{w_1,w_2\}$ where $w_1,w_2$ are square vertices, and $E(\alpha_{1}) = \{\{u,w_1\}, \{u,w_2\}, \{w_1,v\},\{w_2,v\}\}$.
    \item $U_{\alpha_{2}} = (u)$ and  $V_{\alpha_{2}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{2}} = \{w\}$ where $w$ is a square vertex, and $E(\alpha_{2}) = \{\{u,w\}, \{u,w\}, \{w,v\},\{w,v\}\}$.
    \item $U_{\alpha_{3}} = V_{\alpha_{3}} = (u)$ where $u$ is a circle vertex, $W_{\alpha_{3}} = \{w_1,w_2\}$ where $w_1,w_2$ are square vertices, and $E(\alpha_{3}) = \{\{u,w_1\}, \{u,w_1\}, \{u,w_2\}, \{u,w_2\}\}$.
    \item $U_{\alpha_{4}} = V_{\alpha_{4}} = (u)$ where $u$ is a circle vertex, $W_{\alpha_{4}} = \{w\}$ where $w$ is a square vertex, and $E(\alpha_{4}) = \{\{u,w\}, \{u,w\}, \{u,w\},\{u,w\}\}$.
\end{enumerate}
Insert picture here

To shift from improper shapes to proper shapes, we make the following observations:
\begin{enumerate}
    \item $x^2 = (x^2 - 1) + 1 = \sqrt{2}h_2(x) + 1$
    \item $x^4 = (x^4 - 6x^2 + 3) + 6(x^2 - 1) + 3 = \sqrt{24}h_4(x) + 6\sqrt{2}h_2(x) + 3$
\end{enumerate}
We now have that 
\begin{align*}
{\calA}{\calA}^{*} &= M_{\alpha_1} + 2M_{\alpha_{2a}} + \sqrt{2}M_{\alpha_{2b}} + \sqrt{2}M_{\alpha_{2c}} + dM_{\alpha_{2d}} + 2M_{\alpha_{3a}} + 2\sqrt{2}(d-1)M_{\alpha_{3b}} + (d^2 - d)M_{\alpha_{3c}} \\
&+ \sqrt{24}M_{\alpha_{4}} + 6\sqrt{2}M_{\alpha_{3b}} + 3dM_{\alpha_{3c}}   
\end{align*}
where $\alpha_1$, $\alpha_{2a}$, $\alpha_{2b}$, $\alpha_{2c}$, $\alpha_{2d}$, $\alpha_{3a}$, $\alpha_{3b}$, $\alpha_{3c}$, and $\alpha_{4}$ are the following proper shapes:
\begin{enumerate}
    \item $\alpha_1$ is the same as above.
    \item $U_{\alpha_{2a}} = (u)$ and  $V_{\alpha_{2a}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{2a}} = \{w\}$ where $w$ is a square vertex, and $E(\alpha_{2a}) = \{\{u,w\}_2, \{w,v\}_2\}$.
    \item $U_{\alpha_{2b}} = (u)$ and  $V_{\alpha_{2b}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{2b}} = \{w\}$ where $w$ is a square vertex, and $E(\alpha_{2b}) = \{\{u,w\}_2\}$.
    \item $U_{\alpha_{2c}} = (u)$ and  $V_{\alpha_{2c}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{2c}} = \{w\}$ where $w$ is a square vertex, and $E(\alpha_{2c}) = \{\{w,v\}_2\}$.
    \item $U_{\alpha_{2d}} = (u)$ and  $V_{\alpha_{2d}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{2d}} = \{\}$, and $E(\alpha_{2d}) = \{\}$.
    \item $U_{\alpha_{3a}} = V_{\alpha_{3a}} = (u)$ where $u$ is a circle vertex, $W_{\alpha_{3a}} = \{w_1,w_2\}$ where $w_1,w_2$ are square vertices, and $E(\alpha_{3a}) = \{\{u,w_1\}_2, \{u,w_2\}_2\}$.
    \item $U_{\alpha_{3b}} = V_{\alpha_{3a}} = (u)$ where $u$ is a circle vertex, $W_{\alpha_{3b}} = \{w\}$ where $w$ is a square vertex, and $E(\alpha_{3b}) = \{\{u,w\}_2\}$.
    \item $U_{\alpha_{3c}} = V_{\alpha_{3c}} = (u)$ where $u$ is a circle vertex, $W_{\alpha_{3c}} = \{\}$, and $E(\alpha_{3c}) = \{\}$.
    \item $U_{\alpha_{4}} = V_{\alpha_{4}} = (u)$ where $u$ is a circle vertex, $W_{\alpha_{4}} = \{w\}$ where $w$ is a square vertex, and $E(\alpha_{4}) = \{\{u,w\}_4\}$.
\end{enumerate}
Insert picture here.

Since $M_{\alpha_{2d}} = 1_{n}1_{n}^T - Id_n$ and $M_{\alpha_{3c}} = Id_n$, we have that 
\[
{\calA}{\calA}^{*} = (d^2 + d)Id_{n} + d{1_n}{1_n^T} + M_{\alpha_1} + 2M_{\alpha_{2a}} + \sqrt{2}M_{\alpha_{2b}} + \sqrt{2}M_{\alpha_{2c}} + 2M_{\alpha_{3a}} + (2\sqrt{2}d + 4\sqrt{2})M_{\alpha_{3b}} + \sqrt{24}M_{\alpha_{4}}
\]
Since $M = (d^2 + d)Id_{n} + d{1_n}{1_n}^T$, 
\[
\Delta = M - {\calA}{\calA}^{*} = -M_{\alpha_1} - 2M_{\alpha_{2a}} - \sqrt{2}M_{\alpha_{2b}} - \sqrt{2}M_{\alpha_{2c}} - 2M_{\alpha_{3a}} - (2\sqrt{2}d + 4\sqrt{2})M_{\alpha_{3b}} - \sqrt{24}M_{\alpha_{4}}
\]
\subsection{Computing $M^{-1}\Delta$}
Since $M = (d^2 + d)Id + d{1_n}{1_n}^T$, we have that $M^{-1} = \frac{1}{d^2 + d}\left(Id - \frac{1}{n + d + 1}{1_n}{1_n}^T\right)$.
\begin{definition}
Define $\alpha_J$ to be the shape with $U_{\alpha_J} = (u)$, $V_{\alpha_J} = (v)$, $W_{\alpha_J} = \emptyset$, and $E(\alpha_J) = \emptyset$.
\end{definition}
Since ${1_n}{1_n}^T = Id + M_{\alpha_J}$, we have that 
\[
M^{-1} = \frac{1}{d^2 + d}\left(\frac{n+d}{n+d+1}Id - \frac{1}{n + d + 1}M_{\alpha_J}\right)
\]
We now compute the product of $M_{\alpha_J}$ with each of the graph matrices appearing in $\Delta$.
\begin{enumerate}
    \item $M_{\alpha_J}M_{\alpha_1} = M_{\alpha_5} + M_{\alpha_1}$ where $M_{\alpha_5}$ is the shape such that $U_{\alpha_{5}} = (u)$ and  $V_{\alpha_{5}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{5}} = \{w_{\circ},w_1,w_2\}$ where $w_{\circ}$ is a circle vertex and $w_1,w_2$ are square vertices, and $E(\alpha_{1}) = \{\{w_{\circ},w_1\}, \{w_{\circ},w_2\}, \{w_1,v\},\{w_2,v\}\}$.
    \item $M_{\alpha_J}M_{\alpha_{2a}} = M_{\alpha_{6a}} + M_{\alpha_{2a}}$ where $M_{\alpha_{6a}}$ is the shape such that $U_{\alpha_{6a}} = (u)$ and $V_{\alpha_{6a}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{6a}} = \{w_{\circ},w\}$ where $w_{\circ}$ is a circle vertex and $w$ is a square vertex, and $E(\alpha_{6a}) = \{\{w_{\circ},w\}_2, \{w,v\}_2\}$.
    \item $M_{\alpha_J}M_{\alpha_{2b}} = M_{\alpha_{6b}} + M_{\alpha_{2c}}$ where $M_{\alpha_{6b}}$ is the shape such that $U_{\alpha_{6b}} = (u)$ and $V_{\alpha_{6b}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{6b}} = \{w_{\circ},w\}$ where $w_{\circ}$ is a circle vertex and $w$ is a square vertex, and $E(\alpha_{6b}) = \{\{w_{\circ},w\}_2\}$.
    \item $M_{\alpha_J}M_{\alpha_{2c}} = (n-2)M_{\alpha_{2c}} + M_{\alpha_{2b}}$.
    \item $M_{\alpha_J}M_{\alpha_{3a}} = M_{\alpha_{7a}}$
    where $M_{\alpha_{7a}}$ is the shape such that $U_{\alpha_{7a}} = (u)$ and $V_{\alpha_{7a}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{7a}} = \{w_1,w_2\}$ where $w_1,w_2$ are square vertices, and $E(\alpha_{7a}) = \{\{v,w_1\}_2, \{v,w_2\}_2\}$.
    \item $M_{\alpha_J}M_{\alpha_{3b}} = M_{\alpha_{7b}}$
    where $M_{\alpha_{7b}}$ is the shape such that $U_{\alpha_{7b}} = (u)$ and $V_{\alpha_{7b}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{7b}} = \{w\}$ where $w$ is a square vertex, and $E(\alpha_{7b}) = \{\{v,w\}_2\}$.
    \item $M_{\alpha_J}M_{\alpha_{4}} = M_{\alpha_{8}}$
    where $M_{\alpha_{8}}$ is the shape such that $U_{\alpha_{8}} = (u)$ and $V_{\alpha_{8}} = (v)$ where $u, v$ are circle vertices, $W_{\alpha_{8}} = \{w\}$ where $w$ is a square vertex, and $E(\alpha_{8}) = \{\{v,w\}_4\}$.
\end{enumerate}
Insert pictures here.

Putting everything together, we have that 
\begin{align*}
    M^{-1}\Delta = &\frac{1}{(d^2 + d)(n + d + 1)}\Big(-(n+d)M_{\alpha_1} + \left(M_{\alpha_5} + M_{\alpha_1}\right) -2(n+d)M_{\alpha_{2a}} + 2\left(M_{\alpha_{6a}} + M_{\alpha_{2a}}\right)\\
    &-\sqrt{2}(n+d)M_{\alpha_{2b}} + \sqrt{2}\left(M_{\alpha_{6b}} + M_{\alpha_{2c}}\right)
    -\sqrt{2}(n+d)M_{\alpha_{2c}} + \sqrt{2}\left((n-2)M_{\alpha_{2c}} + M_{\alpha_{2b}}\right)\\
    &-2(n+d)M_{\alpha_{3a}} + 2M_{\alpha_{7a}} -(2\sqrt{2}d + 4\sqrt{2})(n+d)M_{\alpha_{3b}} + (2\sqrt{2}d + 4\sqrt{2})M_{\alpha_{7b}} \\
    &-\sqrt{24}(n+d)M_{\alpha_{4}} + \sqrt{24}M_{\alpha_{8}}\Big) \\
    =&\frac{1}{(d^2 + d)(n + d + 1)}\Big(-(n+d-1)M_{\alpha_1} -2(n+d-1)M_{\alpha_{2a}}
    -\sqrt{2}(n+d-1)M_{\alpha_{2b}}\\
    &-\sqrt{2}(d-1)M_{\alpha_{2c}} -2(n+d)M_{\alpha_{3a}} -(2\sqrt{2}d + 4\sqrt{2})(n+d)M_{\alpha_{3b}} -\sqrt{24}(n+d)M_{\alpha_{4}}\\
    &+ M_{\alpha_5} + 2M_{\alpha_{6a}}  + \sqrt{2}M_{\alpha_{6b}} + 2M_{\alpha_{7a}}  + (2\sqrt{2}d + 4\sqrt{2})M_{\alpha_{7b}} + \sqrt{24}M_{\alpha_{8}}\Big)
\end{align*}
    Thus, when we decompose $M^{-1}\Delta$ into graph matrices, we have the following graph matrices and coefficients:
    \begin{enumerate}
        \item $M_{\alpha_1}$, $M_{\alpha_{2a}}$, and  $M_{\alpha_{2b}}$ appear with coefficients of magnitude $O(\frac{1}{d^2})$. These terms are significant.
        \item $M_{\alpha_{2c}}$ appears with a coefficient of magnitude $O(\frac{1}{dn})$. This term is also significant.
        \item $M_{\alpha_{3a}}$ and $M_{\alpha_{4}}$ appear with coefficients of magnitude $O(\frac{1}{d^2})$. These are lower order terms.
        \item $M_{\alpha_{3b}}$ appears with a coefficient of magnitude $O(\frac{1}{d})$. This is a lower order term.
        \item $M_{\alpha_5}$, $M_{\alpha_{6a}}$,  $M_{\alpha_{6b}}$, $M_{\alpha_{7a}}$, and $M_{\alpha_8}$ appear with coefficients of magnitude $O(\frac{1}{d^2{n}})$. These are lower order terms.
        \item $M_{\alpha_{7b}}$ appears with a coefficient of magnitude $O(\frac{1}{dn})$. This is also a lower order term.
    \end{enumerate}

==> Notes/pax_macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%environments
 \newtheorem{theorem}{Theorem}
 \newtheorem{claim}{Claim}
 \newtheorem{assumption}{Assumption}
 \newtheorem{lemma}{Lemma}
 \newtheorem{problem}{Problem}
 \newtheorem{proposition}{Proposition}
 \newtheorem{corollary}{Corollary}
 \newtheorem{remark}{Remark}
 \newtheorem{definition}{Definition}
 \newtheorem{conjecture}{Conjecture}
\newtheorem{question}{Question}
 \newtheorem{algorithm}{Algorithm}
%\newtheorem*{theorem*}{Theorem}
%\newtheorem*{lemma*}{Lemma}
%\newtheorem*{proposition*}{Proposition}
%\newtheorem*{corollary*}{Corollary}

\newenvironment{myalgo}[1]%
{
	\vspace{0.3cm}
	\begin{center}
		\begin{boxedminipage}{0.8\linewidth}
			\begin{center}
				\textbf{\texttt{#1}}
			\end{center}
			\rm
			\begin{tabbing}
				....\=...\=...\=...\=...\=  \+ \kill
			} %
			{\end{tabbing}
	\end{boxedminipage} \end{center} %\vspace{0.3cm}
}

%%%%%%%%%%%%%% shorthand commands
\newcommand{\flo}[1]{\lfloor #1 \rfloor} %floor
\newcommand{\ceil}[1]{\lceil #1 \rceil} %ceiling
\newcommand{\eps}{\varepsilon} %epsilon
\newcommand{\vp}{\varphi} %varphi
\newcommand{\supp}{\mathrm{supp}} %support
 \newcommand{\E}{\mathbb{E}} %expectation
\newcommand{\ee}{\mathbb{E}} %in-line expectation
\newcommand{\ov}[1]{\overline{#1}} %overline
\newcommand{\mb}[1]{\mathbb{#1}} %blackboard bold
\newcommand{\mf}[1]{\mathbf{#1}} %mathbold 
\newcommand{\msf}[1]{\mathsf{#1}} %mathsansserif
\newcommand{\mc}[1]{\mathcal{#1}} %mathcal 
 \newcommand{\rp}[1]{^{(#1)}} %raise to parentheses
 \newcommand{\1}{\mathbbm{1}} %indicator
\newcommand{\X}{\mathbf{X}\,} %bold capital X
\newcommand{\uu}{\mathbf{u}\,} %bold lowercase u
\newcommand{\vv}{\mathbf{v}\,} %bold lowercase v
\newcommand{\x}{\mathbf{x}\,} %bold lowercase x
\newcommand{\y}{\mathbf{y}\,} %bold lowercase y
\newcommand{\z}{\mathbf{z}\,} %bold lowercase z
\newcommand{\sgn}{\text{sgn}} %sign 
\newcommand{\mr}[1]{\mathrm{#1}} %mathrm 
\newcommand{\abs}[1]{\left|#1\right|} %abs
\newcommand{\norm}[1]{\lVert#1\rVert} %norm
\newcommand{\pd}{\mc{P}_{\mc{H}}(\beta)} %Holder probability densities
\newcommand{\V}[1]{^{\vec{#1}} } %raise to vector
\newcommand{\J}{_{\vec{j}} } %underscore to vector j
\newcommand{\I}{[-\frac{1}{2}, \frac{1}{2}]} %sign
\newcommand{\hd}{ \mc{P}_\mc{H} } %Holder density notation
\newcommand{\sd}{ \mc{P}_\mc{S} } %Sobolev density notation
 %Pax notes
 \newcommand{\ud}{\mathrm{d}} %roman d for integrals 
\newcommand{\unif}{\hat f_S^{\mathsf{unif}}} %uniform weighted coreset
 \newcommand{\cbeta}{\lfloor \beta \rfloor} %floor of beta
\newcommand{\Cara}{Carath\'{e}odory } %Caratheodory
\newcommand{\ti}{\widetilde } %tilde 
\newcommand{\disc}{\mathsf{disc} } %discrepancy

 \newcommand{\cA}{\mathcal{A}}
 \newcommand{\cB}{\mathcal{B}}
 \newcommand{\cC}{\mathcal{C}}
 \newcommand{\cD}{\mathcal{D}}
 \newcommand{\cE}{\mathcal{E}}
 \newcommand{\cF}{\mathcal{F}}
 \newcommand{\cG}{\mathcal{G}}
 \newcommand{\cH}{\mathcal{H}}
 \newcommand{\cI}{\mathcal{I}}
 \newcommand{\cJ}{\mathcal{J}}
 \newcommand{\cK}{\mathcal{K}}
 \newcommand{\cM}{\mathcal{M}}
 \newcommand{\cN}{\mathcal{N}}
 \newcommand{\cO}{\mathcal{O}}
 \newcommand{\cP}{\mathcal{P}}
 \newcommand{\cQ}{\mathcal{Q}}
 \newcommand{\cS}{\mathcal{S}}
 \newcommand{\cT}{\mathcal{T}}
 \newcommand{\cU}{\mathcal{U}}
 \newcommand{\cV}{\mathcal{V}}
 \newcommand{\cW}{\mathcal{V}}
 \newcommand{\cX}{\mathcal{X}}
 \newcommand{\cY}{\mathcal{Y}}
 \newcommand{\cZ}{\mathcal{Z}}

\newcommand{\p}{\mb{P}}
\newcommand{\R}{\mb{R}}
\newcommand{\var}{\mathsf{Var}}
\newcommand{\cov}{\mathsf{Cov}}
\newcommand{\om}{\Omega_{ij}}
\newcommand{\omj}{\Omega_{ij}}
\newcommand{\omk}{\Omega_{ik}}
\newcommand{\sig}{\sigma_{ij}}
\newcommand{\sigj}{\sigma_{ij}}
\newcommand{\sigk}{\sigma_{ik}}
\newcommand{\psij}{\psi_{ij}}
\newcommand{\psik}{\psi_{ik}}
\newcommand{\et}{\eta_{j}}
\newcommand{\etj}{\eta_{j}}
\newcommand{\etk}{\eta_{k}}
\newcommand{\thj}{\theta_j}
\newcommand{\thk}{\theta_k}
\newcommand{\Yj}{Y_{ij}}
\newcommand{\Yk}{Y_{ik}}
\newcommand{\etij}{\hat \eta_{\sim i, j }}
\newcommand{\etik}{\hat \eta_{\sim i, k }}
\newcommand{\thij}{\hat \theta_{\sim i, j }}
\newcommand{\thik}{\hat \theta_{\sim i, k}}
\newcommand{\T}{\mathsf{T}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\tr}{\mathrm{Tr}}
\newcommand{\ck}{\check}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\be}{\mathbf{e}}

\newcommand{\oD}{\overline{\Delta}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand\num{\addtocounter{equation}{1}\tag{\theequation}}

==> omit.tex <==
\section{Direct approach}
Define the following random variables:
\[
\gamma = \inf_{X \succeq 0} \norm{\mathcal{A}(X) - 1_n}_2,
\]
and
\[
\gamma_{1 \pm o(1)} = \inf_{X \succeq 0, \Tr (X) = 1 \pm o(1)} \norm{\mathcal{A}(X) - 1_n}_2.
\]
Observe that it always holds that $\gamma \leq \gamma_{1 \pm o(1)}$. In fact, the reverse direction effectively holds as well.
\begin{claim}
$\Prob (\gamma_{1 \pm o(1)} > 0) - o(1) \leq \Prob (\gamma > 0).$
\end{claim}
\begin{proof}
Let $E$ be the event that $\frac{1}{n} \sum_{i} v_i v_i^T = (1 \pm o(1)) I_d$. Suppose $\gamma = 0$ and $E$ holds. Then there exists $X \succeq 0$ so that
\[
1 = \frac{1}{n} \sum_i v^T_i X v_i^T = \ip{X}{\frac{1}{n} \sum_{i} v_i v_i^T} = \ip{X}{(1 \pm o(1)) I_d} = (1 \pm o(1)) \Tr (X).
\]
The contrapositive of the previous statement then implies that 
\[
\Prob(\gamma_{1 \pm o(1)} > 0) \leq \Prob (E^c \cup \gamma > 0) \leq \Prob(E^c) + \Prob (\gamma > 0).
\]
\end{proof}


The following is a simple extension of Proposition 5.1 of \cite{tropp2015convex}.
\begin{claim}
For any $\theta, t > 0$, the following holds with probability at least $1-e^{-t^2/2}$:
\[
\gamma_{1 \pm o(1)} > \theta \sqrt{n} \inf_{X \succeq 0, \Tr (X) = 1 \pm o(1)} Q_{2 \theta} (X) - 2W - \theta t,
\]
where $Q_{2 \theta} (X) = \Prob (|v^T X v - 1| > 2\theta)$ and
\[
W = \frac{1}{\sqrt{n}} \E \sup_{X \succeq 0, \Tr (X) = 1 \pm o(1)} \sum_{i=1}^n \epsilon_i (v_i^T X v_i - 1),
\]
where $\epsilon \sim \Rad (1/2)^{\otimes n}$.
\end{claim}

We now proceed to heuristically estimate when the above claim implies $\gamma_{1 \pm o(1)} > 0$.
\paragraph{Width term $W$}
First, note that
\[
W = \frac{1}{\sqrt{n}} \E \sup_{X \succeq 0, \Tr (X) = 1 \pm o(1)} \sum_{i=1}^n \epsilon_i v_i^T X v_i \leq \frac{1+o(1)}{\sqrt{n}} \E \lambda_{max} \left( \sum_{i=1}^n \epsilon_i v_i v_i^T \right).
\]
We predict that the eigenvalue should scale like the square-root of the norm of matrix variance, which is $\sqrt{dn}$. More precisely, let us assume for now that there is a small constant $\alpha$ (say, $\alpha = 1$) so that 
\[
\E \lambda_{max} \left( \sum_{i=1}^n \epsilon_i v_i v_i^T \right) \leq \alpha \sqrt{dn}.
\]
We remark that a black-box application of an off-the-shelf matrix concentration inequality will lead to some extra $\log (d)$ factors on the right-hand side.

\paragraph{Tail function term}
First, we predict that the $X$ minimizing $Q_{2\theta} (X)$ is $X = \frac{1}{d} I_d$. For this choice of $X$, we have
\[
Q_{2\theta} \left(\frac{1}{d} I_d \right) = \Prob \left( \left|\frac{1}{d} \chi^2_d - 1 \right| > 2\theta \right).
\]
Intuitively, this choice of $X$ seems to make the random variable $v^T X v$ as well concentrated as possible. Given the above, it should be the case that the optimal choice of $\theta$ is $\theta = c/\sqrt{d}$ for some constant $c>0$. Define $p(c) = \Prob(|g| > 2c/\sqrt{d})$ where $g \sim \calN(0, 2/d)$.

\paragraph{Final inequality}
Assembling the heuristics and dropping the $t$-dependent term o the RHS pf the conclusion of the previous claim, we have
\begin{align*}
\gamma_{1 \pm o(1)} &> \theta \sqrt{n} \inf_{X \succeq 0, \Tr (X) = 1 \pm o(1)} Q_{2 \theta} (X) - 2W - \theta t  \\
&\approx \frac{c\sqrt{n} p(c)}{\sqrt{d}} - 2 \alpha \sqrt{d}.
\end{align*}
This latter quantity will be positive provided
\[
n > \frac{4 \alpha^2}{c^2 p(c)^2} d^2.
\]
After numerically computing $cp(c)$ for various values of $c > 0$, it appears that the maximum possible value is approximately $0.25$, which gives roughly $n > 64d^2$. Note that this does not beat the trivial $n > 0.5 d^2$ threshold for infeasibility of the linear constraints alone.


\subsection{Dual}
Re-define $\gamma$ as follows:
\[
\gamma = \inf_{X \succeq 0} \norm{\mathcal{A}(X) - 1_n}_2^2.
\]
Next define the function $g$ as
\[
g(Y) = \inf_{X \in \R^{d \times d}} \norm{\mathcal{A}(X) - 1_n}_2^2 - \ip{X}{Y}
\]
so that $g(Y) \leq \gamma$ for any $Y \succeq 0$. We then have a weak duality:
\[
\sup_{Y \succeq 0} g(Y) \leq \gamma
\]
It also seems reasonable to assume that equality holds (strong duality). If this is indeed the case, then since $\gamma \geq 0$, it suffices to show that $\sup_{Y \succeq 0} g(Y) \leq 0$ in order to conclude that $\gamma = 0$.

We now attempt to simplify the expression for $g(Y)$ so that it might be more tractable to show $\sup_{Y \succeq 0} g(Y) \leq 0$. Computing the gradient, we obtain
\[
\nabla g(Y) = 2 \calA \calA^* (X) - 2\calA^* (1_n) - Y.
\]
Settiing equal to 0 and solving for $X$, we conclude that 
\[
g(Y) = \norm{\mathcal{A}(X) - 1_n}_2^2 - \ip{X}{Y},
\]
for $X = \left( \calA^* \calA \right)^{-1} \left( \calA^* (1_n) + \frac{1}{2} Y \right)$.


\section{Different approach to analyzing Saunderson's construction}
\TODO{Verify we can delete this section}
As before, the goal is to show that $X := \calA^* (\calA \calA^*)^{-1} 1_n \succeq 0$. Let $L > \lambda_{max} (\calA \calA^*)$ and $T \in \N$ be parameters whose exact values we will determine later. For now, recall that $\lambda_{max} (\calA \calA^*) \leq \lambda_{max} (M) + \norm{\Delta} \leq dn + O(\sqrt{d}n) = (1+o(1))dn$. We have that:
\begin{align*}
X &= \calA^* (\calA \calA^*)^{-1} 1_n \\
&= \frac{1}{L} \calA^* ( \frac{1}{L }\calA \calA^*)^{-1} 1_n \\
&= \frac{1}{L} \calA^* (I_n - ( I_n - \frac{1}{L}\calA \calA^*))^{-1} 1_n \\
&= \frac{1}{L} \calA^* \left(\sum_{i=0}^\infty (I_n - \frac{1}{L}\calA \calA^*)^i \right) 1_n \\
&= \frac{1}{L} \calA^* \left(I + \sum_{i=1}^T (I_n - \frac{1}{L}\calA \calA^*)^i + \sum_{i=T+1}^\infty (I_n - \frac{1}{L}\calA \calA^*)^i \right) 1_n \\
&\succeq \frac{1}{L} \left( \calA^*(1_n) + \calA^* \sum_{i=1}^T (I_n - \frac{1}{L}\calA \calA^*)^i 1_n - \norm{\calA^* \sum_{i=T+1}^\infty (I_n - \frac{1}{L}\calA \calA^*)^i 1_n} I_n \right).
\end{align*}

To complete the proof that $X \succeq 0$, we would ideally show the following:
\begin{enumerate}
    \item $\sigma_{min} (\calA^* (1_n)) = \sigma_{min}( \sum_{i=1}^n v_i v_i^T) \geq \Omega(n)$. This is an already established fact.
    \item The vector $c = \sum_{i=1}^T (I_n - \frac{1}{L}\calA \calA^*)^i 1_n$ is coordinate-wise non-negative. This will ensure that $\calA^* (c) \succeq 0$. While this a strong statement that might not actually be true, the calculations yield some insight on what the vectors $(I_n - \frac{1}{L}\calA \calA^*)^i 1_n$ actually look like. Even if this statement ends up being false, it might still be possible to control these terms in a way that allows us to complete the proof.
    \item $\norm{\calA^* \sum_{i=T+1}^\infty (I_n - \frac{1}{L}\calA \calA^*)^i 1_n} \leq o(n)$.
\end{enumerate}

\paragraph{Remaining terms of the power series}
Here, we show that $\norm{\calA^* \sum_{i=T+1}^\infty (I_n - \frac{1}{L}\calA \calA^*)^i 1_n} \leq o(n)$.
\begin{claim}
With high probability,
\[
\norm{I - \frac{1}{L} \calA \calA^*} \leq (1- \frac{d^2}{L} + \frac{1}{L}) + \Theta(\frac{n \sqrt{d}}{L}). 
\]
In particular, if $n << d^{3/2}$, then $\norm{I - \frac{1}{L} \calA \calA^*} \leq 1 - \Theta(\frac{d^2}{L})$.
\end{claim}
\begin{proof}
\[
\norm{I - \frac{1}{L} \calA \calA^*} \leq \norm{I - \frac{1}{L} M} + \frac{1}{L} \norm{\Delta} \leq  \norm{I - \frac{1}{L} M} + \Theta(\frac{n \sqrt{d}}{L}) = (1- \frac{d^2}{L} + \frac{1}{L}) + \Theta(\frac{n \sqrt{d}}{L}),
\]
where the last step follows from the fact that 
\[
I - \frac{1}{L} M = (1- \frac{d^2}{L} + \frac{1}{L}) (I_n - \frac{1}{n} 11^T) + (1- \frac{d^2}{L} - \frac{dn}{L} + \frac{d}{L})\frac{1}{n} 11^T
\]
\end{proof}
The main takeaway is that we can now bound the contribution of the remaining terms of the series:
\begin{align*}
\norm{\calA^* \sum_{i=T+1}^\infty (I_n - \frac{1}{L}\calA \calA^*)^i 1_n} &\leq \norm{\calA^*}_{2 \rightarrow op} \left( \sum_{i=T+1}^\infty \norm{I - \frac{1}{L} \calA \calA^*}^i_{op} \right) \norm{1_n}_2 \\
\lesssim \sqrt{n} \cdot (1-\frac{d^2}{L})^T \cdot \sqrt{n}.
\end{align*}
So, if $n << d^{3/2}$, we require $T \geq \Omega(\frac{L}{d^2})$ for these terms to contributed at most $\epsilon n$ for a small constant $\epsilon > 0$.

\paragraph{Non-negativity of $c$}
We will attempt to show that for any $i \leq T$, $(I_n - \frac{1}{L}\calA \calA^*)^i 1_n$ is coordinate-wise non-negative. From the previous paragraph, we know that we must be able to handle $T \geq \Omega(\frac{L}{d^2})$ (for the regime $n << d^{3/2}$).

We begin with the case $i=1$. The vector $(I_n - \frac{1}{L}\calA \calA^*) 1_n$ has identically distributed coordinates, the first of which is:
\[
((I_n - \frac{1}{L}\calA \calA^*) 1_n)_1 = 1 - \frac{1}{L} \sum_{i=1}^n \ip{v_1}{v_i}^2 \approx 1- \frac{1}{L} \left( (d \pm \Theta (\sqrt{d}))^2 + (n-1) (\pm \Theta \sqrt{d})^2\right)
\]
We see that the effect of applying $(I_n - \frac{1}{L}\calA \calA^*)$ is that it shrinks the coordinates of $1_n$. If we repeatedly apply it, the coordinates will become negative. We can prevent this from happening by choosing $L$ to be large. On the other hand, choosing $L$ large will make $T$ larger, which requires us to control more terms. In the ideal case, we would be able to choose $L$ so that by the time  $(I_n - \frac{1}{L}\calA \calA^*)^i 1_n$ has negative coordinates, $i > T$ and we can disregard its contribution. Unfortunately, this turns out not to be the case. (For example, one can easily verify the particular cases $L = \Theta (dn)$ does not work.)


